Position-aware Graph Neural Networks

Learning node embeddings that capture a node's position within the broader graph structure is crucial for many prediction tasks on graphs. However, existing Graph Neural Network (GNN) architectures have limited power in capturing the position/location of a given node with respect to all other nodes of the graph. Here we propose Position-aware Graph Neural Networks (P-GNNs), a new class of GNNs for computing position-aware node embeddings. P-GNN first samples sets of anchor nodes, computes the distance of a given target node to each anchor-set,and then learns a non-linear distance-weighted aggregation scheme over the anchor-sets. This way P-GNNs can capture positions/locations of nodes with respect to the anchor nodes. P-GNNs have several advantages: they are inductive, scalable,and can incorporate node feature information. We apply P-GNNs to multiple prediction tasks including link prediction and community detection. We show that P-GNNs consistently outperform state of the art GNNs, with up to 66% improvement in terms of the ROC AUC score.

==> Position-aware Graph Neural Networks (1)/000abstract.tex <==
Learning node embeddings that capture a node's position within the broader graph structure is crucial for many prediction tasks on graphs.
However, existing Graph Neural Network (GNN) architectures have limited power in capturing the position/location of a given node with respect to all other nodes of the graph.
Here we propose {\em Position-aware Graph Neural Networks (P-GNNs)}, a new class of GNNs for computing position-aware node embeddings. P-GNN first samples sets of anchor nodes, computes the distance of a given target node to each anchor-set, and then learns a non-linear distance-weighted aggregation scheme over the anchor-sets. This way P-GNNs can capture positions/locations of nodes with respect to the anchor nodes.
P-GNNs have several advantages: they are inductive, scalable, and can incorporate node feature information.
We apply P-GNNs to multiple prediction tasks including link prediction and community detection. We show that P-GNNs consistently outperform state of the art GNNs, with up to 66\% improvement in terms of the ROC AUC score.

%% Old (Jan 21)
\cut{
Learning node embeddings that are aware of the position of nodes within a graph is crucial for many prediction tasks such as node classification, link prediction, and community detection.
However, while expressive and most popular, existing Graph Neural Network (GNN) approaches have limited power for representing positions/locations of nodes in a bigger network structure.
%, and can only capture structural information of nodes in most cases.
Here we propose {\em Position-aware Graph Neural Networks (P-GNN)}, a new class of GNNs for computing position-aware node embeddings and remains inductive, via computing shortest path based distances between a node and randomly selected node subsets.
We apply P-GNN to multiple prediction tasks including link prediction and community detection. We show that both variants of P-GNN consistently outperforms state of the art GNN variants by 20\% in transductive settings, while significantly outperforms GNN models in inductive settings by 50\%. 
}

==> Position-aware Graph Neural Networks (1)/010intro.tex <==
\section{Introduction}

Learning low-dimensional vector representations of nodes in graphs \cite{hamilton2017representation} has led to advances on tasks such as node classification \cite{kipf2016semi}, link prediction \cite{grover2016node2vec}, graph classification \cite{ying2018hierarchical} and graph generation \cite{you2018graphrnn}, with successful applications across domains such as social and information networks \cite{ying2018graph}, chemistry \cite{you2018graph}, and biology \cite{zitnik2017predicting}.

Node embedding methods can be categorized into Graph Neural Networks (GNNs) approaches \cite{scarselli2009graph}, matrix-factorization approaches \cite{belkin2002laplacian}, and random-walk approaches \cite{perozzi2014deepwalk}. Among these, GNNs are currently the most popular paradigm, largely owing to their efficiency and inductive learning capability~\cite{hamilton2017inductive}. By contrast, random-walk approaches~\cite{perozzi2014deepwalk,grover2016node2vec} are limited to transductive settings and cannot incorporate node attributes. In the GNN framework, the embedding of a node is computed by a GNN layer aggregating information from the node's network neighbors via non-linear transformation and aggregation functions~\cite{battaglia2018relational}. Long-range node dependencies can be captured via stacking multiple GNN layers, allowing the information to propagate for multiple-hops~\cite{xu2018representation}. 
% \jure{sprinkle more citations here}


% TODO: define position-aware more explicitly
However, the key limitation of existing GNN architectures is that they fail to capture the {\em position/location} of the node within the broader context of the graph structure. 
For example, if two nodes reside in very different parts of the graph but have topologically the same (local) neighbourhood structure, they will have identical GNN structure. Therefore, the GNN will embed them to the same point in the embedding space (we ignore node attributes for now). Figure~\ref{fig:example} gives an example where a GNN cannot distinguish between nodes $v_1$ and $v_2$ and will always embed them to the same point because they have isomorphic network neighborhoods. Thus, GNNs will never be able to classify nodes $v_1$ and $v_2$ into different classes because from the GNN point of view they are indistinguishable (again, not considering node attributes).
%
% Figure \ref{fig:example} illustrates tasks like link prediction \CITE and community detection \CITE where node positional information is crucial, but GNNs will fail due to only capturing a node's structural information.
% \jure{We can shorten/cut the following text or expand it to mention other methods --- like deep GCNs and other work and could potentially solve this proble. We need lots of citations.}
Researchers have spotted this weakness~\cite{xu2018powerful} and developed heuristics to fix the issue: augmenting node features with one-hot encodings \cite{kipf2016semi}, or making GNNs deeper~\cite{selsam2018learning}. However, models trained with one-hot encodings cannot generalize to unseen graphs, and arbitrarily deep GNNs still cannot distinguish structurally isomorphic nodes (Figure \ref{fig:example}).
% and a GNN model is required to learn from exponential number of node permutations in order to generalize to unseen graphs.
% this approach makes the learned model transductive, i.e., the learned GNN model can neither adapt to the same graph with permuted node ordering, nor it can adapt to unseen graphs.
% In applications, learning node embeddings that are aware of node positions in graphs is crucial for many graph prediction tasks, as it can lead to better predictive performance and more faithful embeddings.
% , \jure{we need to be more explicit why position is useful for these tasks. Give an example, why this is advantageous} For example, tasks like link prediction \CITE, community detection \CITE, and node classification \CITE can all benefit from more accurately capturing node's location inside a big network. 
%. however, this aspect has not yet raised enough attention in the design of graph neural networks.

% \jiaxuan{OK! I have an illustrative example, I'll add it here.}
\begin{figure}
    \centering
    \includegraphics[width=0.42\textwidth]{figs/example.png}
    \caption{Example graph where GNN is not able to distinguish and thus classify nodes $v_1$ and $v_2$ into different classes based on the network structure alone. (Note we do not consider node features.)
    Each node is labeled based on its label $A$ or $B$, and effective node embedding should be able to learn to distinguish nodes $v_1$ and $v_2$ (that is, embed them into different points in the space). However, GNNs, regardless of depth, will \textit{always} assign the same embedding to both nodes,
    % (without the help of node features)
    because the two nodes are symmetric/isomorphic in the graph, and their GNN rooted subtrees used for message aggregation are the same. In contrast, P-GNNs can break the symmetry by using $v_3$ as the anchor-set, then the shortest path distances $(v_1, v_3)$ and $(v_2, v_3)$ are different and nodes $v_1$ and $v_2$ can thus be distinguished.
    }
    \label{fig:example}
\vspace{-3mm}
\end{figure}

Here we propose {\em Position-aware Graph Neural Networks (P-GNNs)}, a new class of Graph Neural Networks for computing node embeddings that incorporate a node's positional information with respect to all other nodes in the network, while also retaining inductive capability and utilizing node features.
Our key observation is that node position can be captured by a low-distortion embedding by quantifying the distance between a given node and a set of anchor nodes.
Specifically, P-GNN uses a sampling strategy with theoretical guarantees to choose $k$ random subsets of nodes called {\em anchor-sets}. %and  to compute a $k$-dimensional distance vector to all anchor sets. 
To compute a node's embedding, P-GNN first samples multiple anchor-sets in each forward pass, then learns a non-linear aggregation scheme that combines node feature information from each anchor-set and weighs it by the distance between the node and the anchor-set. Such aggregations can be naturally chained and combined into multiple layers to enhance model expressiveness.
%computes the representation based on the estimated distance between the node and the anchor set, \jure{unclear:} and then applies non-linear transformation via multiple layers to enhance expressiveness and incorporate feature information. 
Bourgain theorem \cite{bourgain1985lipschitz} guarantees that only $k = O(\log^2 n)$ anchor-sets are needed to preserve the distances in the original graph with low distortion. %, where $n$ is the number of nodes.

We demonstrate the P-GNN framework in various real-world graph-based prediction tasks. In settings where node attributes are not available, P-GNN's computation of the $k$ dimensional distance vector is inductive across different node orderings and different graphs.
%In addition, P-GNN can make use of node attributes as well. 
When node attributes are available, a node's embedding is further enriched by aggregating information from all anchor-sets, weighted by the $k$ dimensional distance vector.
Furthermore, we show theoretically that P-GNNs are more general and expressive than traditional message-passing GNNs. In fact, message-passing GNNs can be viewed as special cases of P-GNNs with degenerated distance metrics and anchor-set sampling strategies.
In large-scale applications, computing distances between nodes can be prohibitively expensive. Therefore, we also propose P-GNN-Fast which adopts approximate node distance computation. We show that P-GNN-Fast has the same computational complexity as traditional GNN models while still preserving the benefits of P-GNN.

We apply P-GNNs to 8 different datasets and several different prediction tasks including link prediction and community detection\footnote{Code and data are available in \url{https://github.com/JiaxuanYou/P-GNN/}}. In all datasets and prediction tasks, we show that P-GNNs consistently outperforms state of the art GNN variants, with up to 66\% AUC score improvement.




==> Position-aware Graph Neural Networks (1)/020related.tex <==
\section{Related Work}

% \jure{if we are short on space, we can cut/skip related work since we do a good job in the intro already}

% \xhdr{Inductive Graph Neural Networks}
% Inductive learning on graphs means that the same learned model can generalize to the same graph with different node orderings or across different graphs.
% GraphSAGE \cite{hamilton2017inductive} first demonstrated the inductive learning capability of GNNs, and proposes the sampling and aggregation framework for large-scale GNNs.
% The model can be further extended to incorporate attention over neighborhood\CITE, and aggregate over larger neighborhood at each layer.
% SEAL, which is based on pre-trained node2vec features that are transductive \cite{zhang2018link}.

% Although these GNNs models are inductive, they focus on structural equivalence and node features, and fail to capture nodes' positional information within the graph.
% To learn nodes' positional information required in many tasks, a common workaround in these work is to assign an unique identifier to each node, which the tradeoff of losing its inductive learning capability. 
% \name, however, can capture positional information well without sacrificing the other advantages of GNNs.

% \xhdr{Non-local (Graph) Neural Networks}
% Many (graph) neural network variants include non-local information in the design; therefore, the computed node embeddings are aware of global information across the entire graph.
% Non-local neural network, computes pairwise attention weights between all nodes then aggregates the information, directly gaining global information.
% Graph network, a generalize GNN framework, where a global latent embedding is used to update node embeddings.
% Deep Graph Infomax\CITE, where nodes are represented by their local patch representations that are trained to maximize their mutual information with a global graph representation.
% However, all these existing works focus on learning node embeddings that can capture structural equivalence between nodes and are not position-aware. When computing a node embedding, only the global representation and the local representation themselves are used, while the position of the node does not affect the embedding. 

% \xhdr{Graph Neural Networks variants}
Existing GNN models belong to a family of graph message-passing architectures that use different aggregation schemes for a node to aggregate feature messages from its neighbors in the graph: Graph Convolutional Networks use mean pooling \cite{kipf2016semi}; GraphSAGE concatenates the node's feature in addition to mean/max/LSTM pooled neighborhood information \cite{hamilton2017inductive}; Graph Attention Networks aggregate neighborhood information according to trainable attention weights \cite{velickovic2017graph}; Message Passing Neural Networks further incorporate edge information when doing the aggregation \cite{gilmer2017neural}; And, Graph Networks further consider global graph information during aggregation \cite{battaglia2018relational}.
However, all these models focus on learning node embeddings that capture local network structure around a given node. Such models are at most as powerful as the WL graph isomorphism test \cite{xu2018powerful}, which means that they cannot distinguish nodes at symmetric/isomorphic positions in the network (Figure~\ref{fig:example}). That is, without relying on the node feature information, above models will always embed nodes at symmetric positions into same embedding vectors, which means that such nodes are indistinguishable from the GNN's point of view.

%but cannot capture well nodes' positional information within graphs without combining with node attributes that are indicative of their positions.

Heuristics that alleviate the above issues include assigning an unique identifier to each node \cite{kipf2016semi,hamilton2017inductive} or using locally assigned node identifiers plus pre-trained transductive node features \cite{zhang2018link}.
However, such models are not scalable and cannot generalize to unseen graphs where the canonical node ordering is not available. In contrast, P-GNNs can capture positional information without sacrificing other advantages of GNNs.

% Also related to our work here is the recent work on graph kernels,
One alternative method to incorporate positional information is utilizing a graph kernel,
which crucially rely on the positional information of nodes and inspired our P-GNN model.
Graph kernels implicitly or explicitly map graphs to a Hilbert space. 
Weisfeiler-Lehman and Subgraph kernels have
been incorporated into deep graph kernels~\cite{Yan+2015} to capture structural properties of neighborhoods.
\citeauthor{Gae+2003} (\citeyear{Gae+2003})
and \citeauthor{Kas+2003} (\citeyear{Kas+2003}) also proposed
graph kernels based on random walks, which count the number of walks
two graphs have in common~\cite{Sug+2015}.
Kernels based on shortest paths were first proposed in~\cite{Borgwardt2005}.


% \xhdr{Other node embedding methods}
% Random-walk-based models and the Laplacian eigenmaps are also popular in representation learning for graphs.
% As a notable example, Node2vec \CITE encourages nodes appear in the same random walk to have similar node embedding, and is able to explore both structural equivalence and positional information of a node. However, such approaches are inherently \cite{transductive}, and cannot include node attributes. 



%The Laplacian eigenmaps technique explicitly includes node proximity in the objective function, which implies the computed node embedding to be position-aware. However, the approach is also transductive and does not explicitly include node attributes. \rex{i think not necessary and can be merged to the first sentence}

==> Position-aware Graph Neural Networks (1)/030proposed.tex <==
% \section{Proposed Approach}
\section{Preliminaries}
% \jiaxuan{A figure for the model}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/PGNN.png}
    \caption{P-GNN architecture. P-GNN first samples multiple anchor-sets $S = \{S_1, S_2, S_3\}$ of different sizes (\textbf{Left}). Then, position-aware node embeddings $\mb{z}_{v_i}$ are computed via messages $M_{v_i}$ between a given node $v_i$ and the anchor-sets $S_i$ which are shared across all the nodes (\textbf{Middle}). To compute the embedding $\mb{z}_{v_1}$ for node $v_1$, one layer of P-GNN first computes messages via function $F$ and then aggregates them via a learnable function $\textsc{Agg}_M$ over the nodes in each anchor-set $S_i$ to obtain a matrix of anchor-set messages $\mb{M}_{v_1}$. The message matrix $\mb{M}_{v_1}$ is then further aggregated using a learnable function $\textsc{Agg}_S$ to obtain node $v_1$'s message $\mb{h}_{v_1}$ that can be passed to the next level of P-GNN. At the same time a learned vector $\mb{w}$ is used reduce $\mb{M}_{v_1}$ into a fixed-size position-aware embedding $\mb{z}_{v_1}$ which is the output of the P-GNN (\textbf{Right}).
    % where each dimension corresponds to an anchor-set. Thus the dimension of the final embedding $\mb{z}_{v_1}$ equals the number of anchor-sets $k$. 
    % \jure{simplify notation, remove $l$}.
    %Note that each anchor-set $S$ corresponds to a row of $M$, and each column corresponds to \jure{what}.
    % \jure{update symbols $AGG_H is AGG_M$ now, $M becomes F$.}
    }
    \label{fig:PGNN}
% \vspace{-3mm}
\end{figure*}

\subsection{Notation and Problem Definition}
% \jiaxuan{We will make this shorter}
% notation 
A graph can be represented as $G = (\mathcal{V},\mathcal{E})$, where $\mathcal{V} = \{v_1, ..., v_n\}$ is the node set and $\mathcal{E}$ is the edge set. In many applications where nodes have attributes, we augment $G$ with the node feature set $\mathcal{X} = \{\mb{x}_1, ..., \mb{x}_n\}$ where $\mb{x}_i$ is the feature vector associated with node $v_i$. 

Predictions on graphs are made by first embedding nodes into a low-dimensional space which is then fed into a classifier, potentially in an end-to-end fashion. %
Specifically, a node embedding model can be written as a function $f: \mathcal{V} \rightarrow \mathcal{Z}$ that maps nodes $\mathcal{V}$ to $d$-dimensional vectors $\mathcal{Z} = \{\mb{z}_1, ..., \mb{z}_n\}, \mb{z}_i \in \mathbb{R}^d$.
% , which implies a new metric space $S_z = (Z, d_z)$.
%Node-level prediction tasks correspond to a single-node predictive function $y(v_i)$, while edge-level prediction tasks imply a pairwise node predictive function $y(v_i, v_j)$.
%Learning node embedding can then be written as an optimization problem, $\min \mathbb{E}_{(v_i,v_j)\sim E_{train}}[L(||\mb{z}_i - \mb{z}_j||_p, y(v_i,v_j))]$ for edge-level tasks, and $\min \mathbb{E}_{v_i\sim V_{train}}[L(z_i, y(v_i))]$ for node-level tasks, where $L(\cdot, \cdot)$ is a loss function and $||\cdot||_p$ is $l_p$ norm.
% A common additional requirement is that $d_z(\cdot,\cdot)$ should be $l_2$ metric, so that the computed embeddings are interpretable and can be easily used for downstream tasks.
%The above formulation is for transductive learning settings, where models are trained and tested on the same graph. It can be generalized to inductive settings where training and testing are performed on different graphs.
% In the inductive setting, $G$ is viewed as a sample from a class of graphs $G \in \mathbb{G}$. The goal is to learn an underlying objective function $d_y$ that is share among any $G \in \mathbb{G}$, via a shared embedding model $f$ that can take any $G \in \mathbb{G}$ as input.

% \subsection{GNNs fail to learn position-aware embeddings}

\subsection{Limitations of Structure-aware Embeddings}
\label{sc:limitation_structure_aware}
% \jiaxuan{We will make this shorter}
\cut{
We identify two key properties of node embeddings that are of special interests in applications, which we name as \textit{structure-aware} embeddings and \textit{position-aware} embeddings.
Structure-aware embeddings detect the structural role for a given node, usually involve some approximate graph isomorphism test. 
Position-aware embeddings reflect homophily properties in the graph \cite{grover2016node2vec}, which is highly related to the shortest path distance metrics.
Usually, tasks such as community detection and link prediction require more of position-aware embeddings, while common node classification tasks reflect more of structure-aware distances \CITE.
Although both types of embeddings have been used to qualitatively discuss the nature of various network prediction tasks, their relationship is not clearly understood. 
}
%We first define two key properties of node embeddings, namely structure-awareness and position-awareness, and demonstrate example models capable of incorporating each property respectively.

Our goal is to learn embeddings that capture the local network structure as well as retain the global network position of a given node.
We call node embeddings to be {\em position-aware}, if the embedding of two nodes can be used to (approximately) recover their shortest path distance in the network. This property is crucial for many prediction tasks, such as link prediction and community detection.
% Specifically, let $d_{sp}(v_i,v_j)$ be the shortest path, then $d_{sp}(v_i, v_j) = g(d_z(f(v_i), f(v_j)))$ holds for position-aware node embeddings. \jure{this is confusing, what is $g$?}
We show below that GNN-based embeddings cannot recover shortest path distances between nodes, which may lead to suboptimal performance in tasks where such information is needed.

\begin{definition}
A node embedding $\mb{z}_i = f_p(v_i), \forall v_i \in \mathcal{V}$ is position-aware if there exists a function $g_p(\cdot, \cdot)$ such that $d_{sp}(v_i, v_j) = g_p(\mb{z}_i, \mb{z}_j)$, where $d_{sp}(\cdot, \cdot)$ is the shortest path distance in $G$.
\end{definition}

\begin{definition}
A node embedding $\mb{z}_i = f_{s_q}(v_i), \forall v_i \in \mathcal{V}$ is structure-aware if it is a function of up to $q$-hop network neighbourhood of node $v_i$. Specifically, $\mb{z}_i = g_s(N_1(v_i),...,N_q(v_i))$, where $N_k(v_i)$ is the set of the nodes $k$-hops away from node $v_i$, and $g_s$ can be any function.
\end{definition}

For example, most graph neural networks compute node embeddings by aggregating information from each node's $q$-hop neighborhood, and are thus structure-aware. In contrast, (long) random-walk-based embeddings such as DeepWalk and Node2Vec are position-aware, since their objective function forces nodes that are close in the shortest path to also be close in the embedding space. 
%Based on the definitions, we point out that there is a dichotomy between structure-aware and position-aware embeddings. 
In general, structure-aware embeddings cannot be mapped to position-aware embeddings.
Therefore, when the learning task requires node positional information, only using structure-aware embeddings as input is not sufficient:

\begin{proposition}
\label{prop:emb_dichoto}
There exists a mapping $g$ that maps structure-aware embeddings $f_{s_q}(v_i), \forall v_i \in \mathcal{V}$ to position-aware embeddings $f_p(v_i), \forall v_i \in \mathcal{V}$, if and only if no pair of nodes have isomorphic local $q$-hop neighbourhood graphs.
\end{proposition}

Proposition \ref{prop:emb_dichoto} is proved in the Appendix. The proof is based on the identifiability arguments similar to the proof of Theorem 1 in \cite{hamilton2017inductive}, and also explains why in some cases GNNs may perform well in tasks requiring positional information. However, in real-world graphs such as molecules and social networks, the structural equivalences between nodes' local neighbourhood graphs are quite common, making GNNs hard to identify different nodes.
% In current literature, 2-layer GNNs are commonly used \cite{hamilton2017inductive}, which corresponds to computing at most 2-hop structure-aware node embeddings.
% However in general, network diameters are generally much bigger than 2 and the structural role of a node thus rarely indicates the position of the node in the network. 
Furthermore, the mapping $g$ essentially memorizes the shortest path distance between a pair of structure-aware node embeddings whose local neighbourhoods are unique. Therefore, even if the GNN perfectly learns the mapping $g$, it cannot generalize to the mapping to new graphs.
% since the GNN needs to memorize each node's identity by its unique neighborhood structure. Therefore, the expressive capacity of structure-aware node embeddings in tasks that require position-aware information is  limited.

\cut{
We concretely state the limitation of structure-aware node embeddings in the inductive setting in Proposition \ref{prop:emb_dichoto_inductive} (proof in the Appendix).


\begin{proposition}
\label{prop:emb_dichoto_inductive}
There does not exist a general mapping $g$ that maps from structure-aware embeddings $f_{s_q}(v_i)$ to shortest path distance $d_{sp}$ for any given graph.
\end{proposition}
}

% As is shown in \CITE, Graph Convolutional Networks (GCNs) are equivalent of doing approximate graph isomorphism test, where $k$-layer GCNs corresponding to computing $d_{s_k}$ at best. Thus, GNN models fail to capture the position-aware component in the objective metric function $d_y(\cdot, \cdot)$. More expressive model is needed to learn the position-aware component in the object.

\cut{
Finally, we point out that while inductive position-aware link-prediction tasks are well-defined and prevalent, inductive position-aware node classification tasks are in fact ill-defined\footnote{Note that position-aware node classification tasks well defined in the transductive setting}.
For different 

In other words, the predictions for position-aware node classification tasks only need to match the node labels \emph{up to permutation of labels}, which is equivalent to link prediction where the links represents the equivalence relation between nodes, and the labels form the quotient set of $V$.

\begin{proposition}
\label{prop:node_transform_edge}
Inductive position-aware node labels are in fact ill-defined. 
There does not exist a position-aware node labeling function for a dataset of multiple graphs, such that the labeling function remains consistent for each input node after permutations of the graphs.
\end{proposition} 
}

\section{Proposed Approach}

In this section, we first describe the \name framework that extends GNNs to learn position-aware node embeddings. We follow by a discussion on our model designing choices. Last, we theoretically show how P-GNNs generalize existing GNNs and learn position-aware embeddings.

\subsection{The Framework of P-GNNs}

We propose Position-aware Graph Neural Networks that generalize the concepts of Graph Neural Networks with two key insights.
First, when computing the node embedding, instead of only aggregating messages computed from a node's local network neighbourhood, we allow P-GNNs to \textit{aggregate messages from anchor-sets}, which are randomly chosen subsets of all the nodes (Figure~\ref{fig:PGNN}, left). 
Note that anchor sets get resampled every time the model is run forward.
% , which grants P-GNNs, with as few as 2 layers, the expressive power to detect any hop graph isomorphism.
Secondly, when performing message aggregation, instead of letting each node aggregate information independently, the aggregation is \textit{coupled across all the nodes} in order to distinguish nodes with different positions in the network (Figure~\ref{fig:PGNN}, middle).
We design P-GNNs such that each node embedding dimension corresponds to messages computed with respect to one anchor-set, which makes the computed node embeddings position-aware (Figure~\ref{fig:PGNN}, right).

%We show later in Section \ref{sc:connection_to_gnns} that existing GNNs can fit nicely into the framework of P-GNNs, while we can enumerate variants of P-GNNs that perform significantly better than existing P-GNNs in the tasks that require position-aware node embeddings.

P-GNNs contain the following key components:\\
\-\hspace{5mm} $\bullet$ $k$ anchor-sets $S_i$ of different sizes.\\
\-\hspace{5mm} $\bullet$ Message computation function $F$ that combines feature information of two nodes with their network distance.\\
\-\hspace{5mm}$\bullet$ Matrix $\mb{M}$ of anchor-set messages, where each row $i$ is an anchor-set message $\mathcal{M}_i$ computed by $F$.\\
\-\hspace{5mm}$\bullet$ Trainable aggregation functions $\textsc{Agg}_M$, $\textsc{Agg}_S$ that aggregate/transform feature information of the nodes in the anchor-set and then also aggregate it across the anchor-sets.\\
\-\hspace{5mm}$\bullet$ Trainable vector $\mb{w}$ that projects message matrix $\mb{M}$ to a lower-dimensional embedding space $\mb{z} \in \mathbb{R}^k$.

Algorithm \ref{alg:pgnn} summarizes the general framework of P-GNNs.
A P-GNN consists of multiple P-GNN layers.
Concretely, the $l^\text{th}$ P-GNN layer first samples $k$ random anchor-sets $S_i$. Then, the $i^{\text{th}}$ dimension of the output node embedding $\mb{z}_{v}$ represents messages computed with respect to the $i^{\text{th}}$ anchor-set $S_i$.
Each dimension of the embedding is obtained by first computing the message from each node in the anchor-set via message computation function $F$, then applying a message aggregation function $\textsc{Agg}_M$, and finally applying a non-linear transformation to get a scalar via weights $\mb{w}\in\mathbb{R}^{r}$ and non-linearity $\sigma$.
Specifically, the message from each node includes distances that reveal node positions as well as feature-based information from input node features. The message aggregation functions are the same class of functions as used by existing GNNs. We further elaborate on the design choices in Section \ref{sc:design_choices}.

\xhdr{P-GNNs are position-aware}
The output embeddings $\mb{z}_v$ are position-aware, as each dimension of the embedding encodes the necessary information to distinguish structurally equivalent nodes that reside in different parts of the graph. Note that if we permute the dimensions of all the node embeddings $\mb{z}_v$, the resulting embeddings are equivalent to the original embeddings because they carry the same node positional information with respect to (permuted order of) anchor-sets $\{S_i\}$.

Multiple P-GNN layers can be naturally stacked to achieve higher expressive power.
Note that unlike GNNs, we cannot feed the output embeddings $\mb{z}_v$ from the previous layer to the next layer, because the dimensions of $\mb{z}_v$ can be arbitrarily permuted; therefore, applying a fixed non-linear transformation over this representation is problematic. The deeper reason we cannot feed $\mb{z}_v$ to the next layer is that the position of a node is always \textit{relative} to the chosen anchor-sets; thus, canonical position-aware embeddings do not exist.
Therefore, P-GNNs also compute structure-aware messages $\mb{h}_{v}$, which are computed via an order-invariant message aggregation function that aggregates messages \textit{across anchor-sets}, and are then fed into the next P-GNN layer as input. 

% We shall show in Section \ref{sc:connection_to_gnns} that existing GNNs can be viewed as P-GNNs that output $\mb{h}_{v}$.

% \begin{algorithm}[h!]
% \caption{The framework of P-GNNs}
% \label{alg:pgnn}
% \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \Input{Graph $G=(\mathcal{V},\mathcal{E})$; 
% %set of anchor-sets $\{S_i, \forall i \in [1,k]\}$;
% Set of $k$ anchor-sets $\{S_i\}$; 
% Node input features $\{\mathbf{x}_v\}$;
% Message computation function $F$ that outputs $r$ dimensional message; 
% Message aggregation functions $\textsc{Agg}_M, \textsc{Agg}_S$;
% Trainable weight vector $\mb{w}\in\mathbb{R}^{r}$;
% Non-linearity $\sigma$;
% % fully connected layer $F^l:  \rightarrow \mathbb{R}^k$; 
% Layer $l \in [1,L]$}
% \Output{Position-aware embedding $\mb{z}_v$ for every node $v$}
% \BlankLine
% $\mathbf{h}_v \leftarrow \mathbf{x}_v$ \\
% \For {$l=1,\dots,L$} {
%     $S_i \sim \mathcal{V}$\- for $i = 1,\dots,k$\\
%     \For {$v \in \mathcal{V}$} {
%         $\mb{M}_v = \mb{0} \in \mathbb{R}^{k\times r}$ \\
%         \For {$i = 1\dots,k$} {
%             $\mathcal{M}_i \leftarrow \{F(v,u,\mb{h}_v,\mb{h}_u),
%             \forall u \in S_i\}$ \\
%             $\mb{M}_v[i] \leftarrow \textsc{Agg}_M(\mathcal{M}_i)$ \\
%         }
%         $\mb{z}_{v} \leftarrow \sigma(\mb{M}_v \cdot \mb{w})$\\
%         $\mb{h}_{v} \leftarrow \textsc{Agg}_S(\{\mb{M}_v[i], \forall i \in [1,k]\})$\\
%     }
%  }
%  $\mb{z}_v \in \mathbb{R}^k$, $\forall v \in \mathcal{V}$ \\
% %  $\mb{h}_v \leftarrow \mb{h}_v^L \in \mathbb{R}^{s_l}$  \\
% \end{algorithm}


\begin{algorithm}[h!]
\caption{The framework of P-GNNs}
\label{alg:pgnn}
\begin{algorithmic}
\STATE {\bfseries Input:} Graph $G=(\mathcal{V},\mathcal{E})$; 
Set $S$ of $k$ anchor-sets $\{S_i\}$; 
Node input features $\{\mathbf{x}_v\}$;
Message computation function $F$ that outputs an $r$ dimensional message; 
Message aggregation functions $\textsc{Agg}_M, \textsc{Agg}_S$;
Trainable weight vector $\mb{w}\in\mathbb{R}^{r}$;
Non-linearity $\sigma$;
Layer $l \in [1,L]$
\STATE {\bfseries Output:} Position-aware embedding $\mb{z}_v$ for every node $v$
\STATE $\mathbf{h}_v \leftarrow \mathbf{x}_v$
\FOR{$l=1,\dots,L$} 
    \STATE $S_i \sim \mathcal{V}$\- for $i = 1,\dots,k$
    \FOR{$v \in \mathcal{V}$} 
        \STATE $\mb{M}_v = \mb{0} \in \mathbb{R}^{k\times r}$ 
        \FOR{$i = 1\dots,k$} 
            \STATE $\mathcal{M}_i \leftarrow \{F(v,u,\mb{h}_v,\mb{h}_u),
            \forall u \in S_i\}$ 
            \STATE $\mb{M}_v[i] \leftarrow \textsc{Agg}_M(\mathcal{M}_i)$ 
        \ENDFOR
        \STATE $\mb{z}_{v} \leftarrow \sigma(\mb{M}_v \cdot \mb{w})$
        \STATE $\mb{h}_{v} \leftarrow \textsc{Agg}_S(\{\mb{M}_v[i], \forall i \in [1,k]\})$
\ENDFOR
\ENDFOR   
 
\STATE $\mb{z}_v \in \mathbb{R}^k$, $\forall v \in \mathcal{V}$ 
%  $\mb{h}_v \leftarrow \mb{h}_v^L \in \mathbb{R}^{s_l}$  \\
\end{algorithmic}
\end{algorithm}



% At every layer, to compute the representation for node $u$, the algorithm first computes representations of all anchor-sets at the previous layer, aggregates them, and passes the aggregated representation along with its own representation at previous layer $\mb{h}_u^{l-1}$ into a non-linear transformation.
% In a message-passing point of view, the message from each anchor-set to node $u$ is a function of the anchor-set representation and the distance between $u$ and the anchor-set.

% The algorithm makes use of $3$ functions. A neighborhood aggregation function $\textsc{Agg}_N$ is used to aggregate representations of neighbors similar to other GNNs. The anchor-set aggregation function $\textsc{Agg}_S(S_i)$ aggregates representations for nodes in the anchor-set $S_i$ and outputs a representation for the anchor-set.
% The distance function $d(\cdot, \cdot)$ measures approximately the distance between a node and an anchor-set. We will discuss design of these functions in the following subsections.

% We emphasize that \name is a general framework for computing position-aware embeddings.
% In general, GNN model can be described by multiple layers of neighborhood aggregations and non-linear transformations \CITE. Therefore different types of GNN with different aggregation functions $\textsc{Agg}_N$ \cite{hamilton2017inductive,velickovic2017graph,battaglia2018relational} can be plugged in to the algorithm to incorporate positional information into embeddings for these models.

% incorporating position info:
% Aggregation per anchor -- set vector, position-aware

% incorporating structure info:
% Aggregation across anchors -- vector, structure-aware; equivalently, GCN aggregation

\subsection{Anchor-set Selection}
\label{sc:anchor_selection}
We rely on Bourgain's Theorem to guide the choice of anchor-sets, such that the resulting representations are guaranteed to have low distortion.
Specifically, distortion measures the faithfulness of the embeddings in preserving distances when mapping from one metric space to another metric space, which is defined as follows:
% Concretely distortion is defined as follows.
\begin{definition}
Given two metric spaces $(\mathcal{V},d)$ and $(\mathcal{Z},d')$ and a function $f: \mathcal{V} \rightarrow \mathcal{Z}$, $f$ is said to have distortion $\alpha$ if $\forall u,v \in \mathcal{V}$, $\frac{1}{\alpha} d(u,v) \leq d'(f(u),f(v)) \leq d(u,v)$.
\end{definition}

Theorem \ref{th:bourgain} states the Bourgain Theorem \cite{bourgain1985lipschitz}, which shows the existence of a low distortion embedding that maps from any metric space to the $l_p$ metric space:
\begin{theorem}
\label{th:bourgain}
(Bourgain theorem)
Given any finite metric space $(\mathcal{V},d)$ with $|\mathcal{V}| = n$, there exists an embedding of $(\mathcal{V}, d)$ into $\mathbb{R}^k$ under any $l_p$ metric, where $k = O(\log^2 n)$, and the distortion of the embedding is $O(\log n)$.
\end{theorem}

A constructive proof of Theorem \ref{th:bourgain} \cite{linial1995geometry} provides an algorithm to construct an $O(\log^2 n)$ dimensional embedding via anchor-sets, as summarized in Theorem \ref{th:bourgain_constructive}:

\begin{theorem}
\label{th:bourgain_constructive}
(Constructive proof of Bourgain theorem)
For metric space $(\mathcal{V},d)$, given $k = c\log^2 n$ random sets $S_{i,j} \subset \mathcal{V}, i=1,2,...,\log n, j = 1,2,...,c\log n$ where $c$ is a constant, $S_{i,j}$ is chosen by including each point in $\mathcal{V}$ independently with probability $\frac{1}{2^i}$. An embedding method for $v \in \mathcal{V}$ is defined as:
\begin{equation}
f(v) = \big( \frac{d(v, S_{1,1})}{k}, \frac{d(v, S_{1,2})}{k}, ..., \frac{d(v, S_{\log n,c\log n})}{k} \big)
\end{equation}
where $d(v, S_{i,j}) = \min_{u\in S_{i,j}} d(v,u)$. Then, $f$ is an embedding method that satisfies Theorem \ref{th:bourgain}.
\end{theorem}

The proposed P-GNNs can be viewed as a generalization of the embedding method in Theorem \ref{th:bourgain_constructive}, where the distance metric $d$ is generalized via message computation function $F$ and message aggregation function $\textsc{Agg}_M$ that accounts for both node feature information and position-based similarities (Section \ref{sc:design_choices}).
Using this analogy, Theorem \ref{th:bourgain_constructive} offers two insights for selecting anchor-sets in P-GNNs. First, $O(\log^2 n)$ anchor-sets are needed to guarantee low distortion embedding. Second, these anchor-sets have sizes distributed exponentially.
Here, we illustrate the intuition behind selecting anchor-sets with different sizes via the $1$-hop shortest path distance defined in Equation~\ref{eq:q_hop_dist}.
Suppose that the model is computing embeddings for node $v_i$. We say an anchor-set \emph{hits} node $v_i$ if $v_i$ or any of its one-hop neighbours is included in the anchor-set. Small anchor-sets can provide positional information with high certainty, because when a small anchor-set hits $v_i$, we know that $v_i$ is located close to one of the very few nodes in the small anchor-set. However, the probability that such small anchor-set hits $v_i$ is low, and the anchor-set is uninformative if it misses $v_i$. On the contrary, large anchor-sets have higher probability of hitting $v_i$, thus sampling large anchor-sets can result in high sample efficiency. However, knowing that a large anchor-set hits $v_i$ provides little information about its position, since $v_i$ might be close to any of the many nodes in the anchor-set.
Therefore, choosing anchor-sets of different sizes balances the trade-off and leads to efficient embeddings.

% \xhdr{Anchor selection}
Following the above principle, P-GNNs choose $k = c\log^2 n$ random anchor-sets, denoted as $S_{i,j} \subset \mathcal{V}$, where $i=1,\dots,\log n, j = 1,\dots,c\log n$ and $c$ is a hyperparameter.
To sample an anchor-set $S_{i,j}$, we sample each node in $\mathcal{V}$ independently with probability $\frac{1}{2^i}$. 

\subsection{Design decisions for P-GNNs}
\label{sc:design_choices}
% Rather than aggregating messages from node neighborhood as in typical GNNs,
% \name aggregates messages from the set of anchor-sets.
% \name computes message from each anchor-set using a distance measure between a node and the anchor-set, in conjunction with the aggregated anchor-set representation.  We demonstrate a family of aggregation functions and effective distance measures.

In this section, we discuss the design choices of the two key components of P-GNNs: the message computation function $F$ and the message aggregation functions $\textsc{Agg}$.
% We then show the specific variant of P-GNN that we develop for the experiments.
% The selection of anchor-sets, which we will discuss later in Section \ref{}

\xhdr{Message Computation Function $F$}
Message computation function $F(v,u,\mb{h}_v,\mb{h}_u)$ has to account for both position-based similarities as well as feature information. Position-based similarities are the key to reveal a node's positional information, while feature information may include other side information that is useful for the prediction task.

Position-based similarities can be computed via the shortest path distance, or, for example, personalized PageRank \cite{jeh2003scaling}. 
However, since the computation of shortest path distances has a $O(|\mathcal{V}|^3)$ computational complexity, we propose the following $q$-hop shortest path distance
% between all pairs of nodes requires computation complexity of $O(|V|^3)$, which restricts its application to real-world graphs which can scale up to billions of nodes \cite{ying2018graph}.
% We show that thresholded shortest path distance can retain the representation power of the shortest path distance, while being computationally efficient. 
% Specifically, a $k$-thresholded shortest path distance can be written as
\begin{equation}
  \label{eq:q_hop_dist}
    d^q_{sp}(v,u) = 
    \begin{cases}
    d_{sp}(v,u),  & \text{if } d_{sp}(v,u) \leq q, \\
    \infty, & \text{otherwise}
    \end{cases}
\end{equation}
where $d_{sp}$ is the shortest path distance between a pair of nodes.
Note that $1$-hop distance can be directly identified from the adjacency matrix, and thus no additional computation is needed. 
Since we aim to map nodes that are close in the network to similar embeddings, we further transform the distance $s(v,u) = \frac{1}{d^q_{sp}(v,u)+1}$ to map it to a $(0,1)$ range.

% To compute $d_{sp}^1$ to random anchors, we describe the following simple algorithm, which we call \textit{coupled neighbourhood sampling}.
% Specifically, we first sample an anchor $S^l$, and each node $v_r \in S^r$ is masked. Then, each node's $1$-thresholded shortest path distance is computed via checking if the nodes connected to it has been masked. The algorithm has complexity of $O(n)$ compared to $O(n^3)$ for exact computation of shortest path distance.

% \xhdr{Feature-based similarity metrics}
Feature information can be incorporated into $\mb{h}_u$ by passing in the information from the neighbouring nodes, as in GCN \cite{kipf2016semi}, or by concatenating node features $\mb{h}_v$ and $\mb{h}_u$, similar to GraphSAGE \cite{hamilton2017inductive}, although other approaches like attention can be used as well \cite{velickovic2017graph}.
Combining position and feature information can then be achieved via concatenation or product. We find that simple product works well empirically. Specifically, we find the following message passing function $F$ performs well empirically
\begin{equation}
   F(v,u,\mb{h}_v,\mb{h}_u) = s(v,u)  \textsc{concat}(\mb{h}_v,\mb{h}_u)
\end{equation}

% can be computed via common functions such as dot product, bi-linear form, or multi-layer perceptron (MLP). We propose to use the following bi-linear form to compute feature-based similarities.
% \begin{equation}
%     d_{bi}(\mb{h}_v^{l-1},\mb{h}_u^{l-1}) = \mb{h}_v^{l-1}\mathbf{W^l}\mb{h}_u^{l-1}
% \end{equation}
% Although these functions do not guarantee that the computed similarities are valid distance metrics, they are shown to be successful in various metric learning settings \cite{koch2015siamese}, and we empirically observe that using similarity between node and anchor-set representations to compute distances, in addition to (thresholded) shortest path, lead to  better model performance. 

% Here we consider the following distance metrics which consistently achieves high performance.

% We use the DeepSet aggregator to aggregate the distance to all elements in the anchor.
% Then, we use either the shortest path distance or $1$ thresholded shortest path distance to include positional information, where $1$ thresholded shortest path distance can be directly computed from the adjacency matrix.

% To compute feature similarity, we use a constant in the settings when node attributes are not available, while using dot product when node attributes are available.

\xhdr{Message Aggregation Functions $\textsc{Agg}$}
% The first design choice is the type of aggregation function to aggregate node representations into an anchor-set representation. 
%In our previous discussion we adopt the $\min$ aggregator $d(x, S) = \min_{y\in S} d(x,y)$. 
% We note that if we choose to measure distance between a node $u$ and an anchor-set $S$ by the shortest path distance between $u$ and the closest node in $S$, then $\min$ is a natural choice.
Message aggregation functions aggregate information from a set of messages (vectors).
Any permutation invariant function, such as $\textsc{Mean}, \textsc{Min}, \textsc{Max}, \textsc{Sum}$, can be used, and non-linear transformations are often applied before and/or after the aggregation to achieve higher expressive power \cite{zaheer2017deep}. 
% We proposed to use $\textsc{Mean}$ based aggregation:
% \begin{equation}
% \begin{aligned}
%     & \textsc{Agg}(\{\mathbf{x}_1,\dots, \mathbf{x}_n\}) = \\
%     & \mathbf{W}_2 \cdot \textsc{Mean}(\{\sigma(\mathbf{W}_1 \cdot \mathbf{x}_i+\mathbf{b}_1 \}) + \mathbf{b}_2
% \end{aligned}
% \end{equation}
% where $\mathbf{W}_1, \mathbf{W}_2, \mathbf{b}_1, \mathbf{b}_2$ are trainable parameters. 
% We use the above function to instantiate both $\textsc{Agg}_M$ and $\textsc{Agg}_S$.
We find that using simple $\textsc{Mean}$ aggregation function provides good results, thus we use it to instantiate both $\textsc{Agg}_M$ and $\textsc{Agg}_S$.


% Overall, the output embedding can be written as:
% \begin{equation}
%     \sigma( \textsc{Mean}(\{\sigma(\mathbf{W}_1 s(v,u)\textsc{Concat}(\mb{h}_v^{l-1},\mb{h}_u^{l-1})+\mathbf{b}_1 , \forall i \in [1,n]\}))
% \end{equation}



% \rex{to be replaced}
% A node embedding vector is computed via both the position-based distance and the feature-based distance
% Then, a node can be represented as a vector where each element is its distance to a random anchor.
% Note that the embedding vectors encode the same information if its dimensions are permuted in the same way for all the nodes, as this operation corresponds to shuffling the order of the random anchors which does not affect the model's expressive power.
% For edge-level prediction tasks, a prediction can be made via directly computing the $l_p$ distance between the two vectors, and the permutation over dimensions does not affect the prediction.

% \subsection{Anchor-set Aggregation}

% For node-level prediction task, we show that unique inductive position-aware node labels are in fact ill-defined. We further show that learning node-level labels can be equivalently transformed into learning edge-level labeling function in Proposition \ref{prop:node_transform_edge} (Proof in appendix \todo{proof}).

% The above formulation emphasizes learning position-aware embeddings, while the structure-aware embeddings are neglected. 
% As we have shown in Proposition \ref{}

\section{Theoretical Analysis of P-GNNs}

\subsection{Connection to Existing GNNs}
\label{sc:connection_to_gnns}
P-GNNs generalize existing GNN models. From P-GNN's point of view, existing GNNs use the same anchor-set message aggregation techniques, but use different anchor-set selection and sampling strategies, and only output the structure-aware embeddings $\mb{h}_{v}$.

GNNs either use deterministic or stochastic neighbourhood aggregation \cite{hamilton2017inductive}.
Deterministic GNNs can be expressed as special cases of P-GNNs that treat each individual node as an anchor-set %(resulting in $|\mathcal{V}|$ anchor-sets), 
and aggregate messages based on $q$-hop distance. In particular, the function $F$ in Algorithm~\ref{alg:pgnn} corresponds to the message aggregation function of a deterministic GNN.
In each layer, most GNNs aggregate information from a node's one-hop neighbourhood \cite{kipf2016semi,velickovic2017graph}, corresponding to using $1$-hop distance to compute messages, or directly aggregating $k$-hop neighbourhood \cite{xu2018representation}, corresponding to computing messages within $k$-hop distance.
For example, a GCN \cite{kipf2016semi} can be written as choosing $\{S_i\} = \{v_i\}$, $\textsc{Agg}_M= \textsc{Mean}$, $\textsc{Agg}_S = \textsc{Mean}$, $F = \frac{1}{d^1_{sp}(v,u)+1}\mb{h}_u$, and the output embedding is $\mb{h}_u$ in the final layer.

Stochastic GNNs can be viewed as P-GNNs that sample size-1 anchor-sets, but each node's choice of anchor-sets is different. For example, GraphSAGE \cite{hamilton2017inductive} can be viewed as a special case of P-GNNs where each node samples $k$ size-1 anchor-sets and then computes messages using 1-hop shortest path distance anchor-set, followed by aggregation $\textsc{Agg}_S$. This understanding reveals the connection between stochastic GNNs and P-GNNs. First, P-GNN uses larger anchor-sets thereby enabling higher sample efficiency (Sec \ref{sc:anchor_selection}).
% Secondly, sampling of anchor-sets is shared across all nodes, such that positional information of each node can be obtained from their distances to anchor-sets which are reference points in the network.
Second, anchor-sets that are shared across all nodes serve as reference points in the network, consequently, positional information of each node can be obtained from the shared anchor-sets.

\subsection{Expressive Power of P-GNNs}
\label{sc:anchor_distance}
Next, we show that P-GNNs provide a more \textit{general class of inductive bias} for graph representation learning than GNNs; therefore, are more expressive to learn both structure-aware and position-aware node embeddings.
% show that a nodes' position-aware embedding can be revealed by computing the shortest path based distance to carefully chosen sets of anchor nodes.
% In fact, we argue that P-GNN is a more expressive class of GNNs, and almost all existing GNNs can be adapted into this model class in order to gain expressiveness in learning position-aware node embeddings.
% We claim that computing the node embedding via computing its shortest path distances to randomly chosen anchors can be both structure-aware and position-aware.
% We define an \textit{anchor} $S \subset V$ to be a random subset of nodes, which is constructed by randomly sampling $l$ nodes from $V$ without replacement.
% Then, we extend the definition of the shortest path distance $d_{sp}$ by defining $d_{sp}(v_i, S^l) = \min_{v_k \in S^l} d_{sp}(v_i, v_k)$.

We motivate our idea by considering pairwise relation prediction between nodes.
Suppose a pair of nodes $u, v$ are labeled with label $y$, using labeling function $d_y(u, v)$, and our goal is to predict $y$ for unseen node pairs.
%If we treat nodes as random variables, then the objective can be written as learning the conditional distribution $p(y|u,v)$.
%then the task corresponds to learning the underlying conditional distribution $p(y|u,v)$, where the labels are generalized to a random variable $Y$, and $U, V \in \mathcal{V}$ are random variables that characterize nodes.
From the perspective of representation learning, we can solve the problem via learning an embedding function $f$ that computes the node embedding $\mb{z}_v$, where the objective is to maximize the likelihood of the conditional distribution $p(y|\mb{z}_u, \mb{z}_v)$. Generally, an embedding function takes a given node $v$ and the graph $G$ as input and can be written as $\mb{z}_v = f(v, G)$, while $p(y|\mb{z}_u, \mb{z}_v)$ can be expressed as a function $d_z(\mb{z}_u, \mb{z}_v)$ in the embedding space.
%Note this is a learning task over euclidean space where mature machine learning techniques can be applied.

%The success of representation learning relies on the \textit{inductive bias} that is chosen for $f_{\theta}$. For example, 
As shown in Section \ref{sc:limitation_structure_aware}, GNNs instantiate $f$ via a function $f_{\theta}(v, S_v)$ that takes a node $v$ and its $q$-hop neighbourhood graph $S_v$ as arguments. Note that $S_v$ is independent from $S_u$ (the $q$-hop neighbourhood graph of node $u$) since knowing the neighbourhood graph structure of node $v$ provides no information on the neighbourhood structure of node $u$.
% However, we also pointed out in Section \ref{sc:limitation_structure_aware} that this function fails to successfully capture the relative position between a pair of nodes in the network.
In contrast, P-GNNs assume a more general type of inductive bias, where $f$ is instantiated via $f_{\phi}(v, S)$ that aggregates messages from random anchor-sets $S$ that are shared across all the nodes, and nodes are differentiated based on their different distances to the anchor-sets $S$. 
Under this formulation, each node's embedding is computed similarly as in the stochastic GNN when combined with a proper $q$-hop distance computation (Section \ref{sc:connection_to_gnns}). However, since the anchor-sets $S$ are shared across all nodes, pairs of node embeddings are correlated via anchor-sets $S$, and are thus no longer independent.
% As we haven shown in Algorithm \ref{alg:pgnn}, the output embedding $\mb{z}_v$ is computed via the message computation function $F$ and the message aggregation functions $\textsc{Agg}$ over anchor-set $S$, which can be generally written as function $f_{\phi}(v, S)$ over $v$ and $S$.
This formulation implies a joint distribution $p(\mb{z}_u, \mb{z}_v)$ over node embeddings, where $\mb{z}_u = f_{\phi}(u, S)$ and $\mb{z}_v = f_{\phi}(v, S)$.
% \cut{Complimentary to the discussion in Section \ref{sc:connection_to_gnns},
% we claim P-GNNs are more general than GNNs.}
%, as the joint distribution $p(\mb{z}_u, \mb{z}_v)$, implies the joint distribution $p(\mb{h}_u, \mb{h}_v)$ over the embeddings $\mb{h}_u, \mb{h}_v$ computed via GNNs.
% \cut{
% \jiaxuan{Firstly, P-GNNs are as expressive as GNNs}, which is summarized in Proposition \ref{prop:marginal_structure}:
% \begin{proposition}
% \label{prop:marginal_structure}
% When using shortest path distances to compute P-GNN messages,
% $p(f_{\phi}(v, S)) = p(f_{\phi}(u, S))$ for $v, u$ if and only if the $\infty$-hop neighbourhood graphs of $v$ and $u$ are isomorphic.
% \end{proposition}
% The proof of Proposition \ref{prop:marginal_structure} is similar to that of Proposition \ref{prop:emb_dichoto} 1 and is given in the Appendix.
% Compared to representations based on marginal distribution (GNNs), the joint distribution $p(\mb{z}_u, \mb{z}_v)$ can also induce position-aware embeddings, as illustrated in Proposition \ref{prop:joint_position}.
% \begin{proposition}
% \label{prop:joint_position}
% The joint distribution $p(f_{\phi}(v, S), f_{\phi}(u, S))$ can reveal nodes' position-aware embeddings, if $f_{\phi}$ is a bijective function of the shortest path distance.
% % The mutual information $I(d_{sp}(V_i, V_j); X_{joint})>0$, where $X_{joint} = (d_{sp}(V_i, S), d_{sp}(V_j, S))$, $(d_{sp}(V_i, S), d_{sp}(V_j, S)) \sim p(d_{sp}(V_i, S), d_{sp}(V_j, S))$.
% \end{proposition}
% Intuitively, the joint distribution of distances between nodes $u$ and $v$ and a common anchor-set  can reveal how similar $u$ and $v$ are in their position, because if both nodes are close to the same anchor-set, they are close to each other in shortest path as well. In contrast, if the marginal distributions are computed independently for $u$ and $v$, then there is no common reference point to infer positional information. 
% }
In summary, \textit{learning node representations} can be formalized with the following two types of objectives:

\-\hspace{5mm} $\bullet$ GNN representation learning objective:
\begin{equation}
\begin{aligned}
\label{eq:ob_edge_marginal}
    \min_\theta & \ \mathbb{E}_{u \sim V_{train}, v \sim V_{train}, S_u \sim p(V) , S_v \sim p(V)} \\
    & \mathcal{L}(d_z(f_{\theta}(u, S_u), f_{\theta}(v, S_v))-d_y(u,v))
\end{aligned}
\end{equation}
\-\hspace{5mm} $\bullet$ P-GNN representation learning objective:
\begin{equation}
\begin{aligned}
\label{eq:ob_edge_joint}
    \min_\theta & \ \mathbb{E}_{u \sim V_{train}, v \sim V_{train}, S \sim p(V)} \\
    & \mathcal{L}(d_z(f_{\phi}(u, S), f_{\phi}(v, S))-d_y(u,v))
\end{aligned}
\end{equation}
where $d_y$ is the target similarity metric determined by the learning task, for example, indicating links between nodes or membership to the same community, and $d_z$ is the similarity metric in the embedding space, usually the $l_p$ norm.

Optimizing Equations \ref{eq:ob_edge_marginal} and \ref{eq:ob_edge_joint} gives representations of nodes using joint and marginal distributions over node embeddings, respectively.
% As shown in Section \ref{sc:connection_to_gnns}, existing stochastic versions of GNNs such as GraphSAGE correspond to learning with objectives in the format of Equation \ref{eq:ob_edge_marginal}, while the proposed P-GNN also learns with objectives in the format of Equation \ref{eq:ob_edge_joint}. 
If we treat $u$, $v$ as random variables from $G$ that can take values of any pair of nodes, 
% by the definition of mutual information,
then the mutual information between the joint distribution of node embeddings and any $Y = d_y(u,v)$ is larger than that between the marginal distributions and $Y$: 
$I(Y; X_{joint}) \geq I(Y; X_{marginal})$, where 
$X_{joint} = (f_{\phi}(u, S_u), f_{\phi}(v, S_v)) \sim p(f_{\phi}(u, S_u), f_{\phi}(v, S_v))$;
$X_{marginal} = (f_{\theta}(u, S), f_{\theta}(v, S)) \sim p(f_{\theta}(u, S)) \otimes p(f_{\theta}(v, S))$, where $\otimes$ is the Kronecker product.
% For example, in the task of representation learning, we can view $Y$ as the random variable between $0$ and $1$ that indicates existence of a link between two nodes, and the joint distribution can better characterize $Y$.  
The gap of this mutual information is great, if the target task $d_y(u,v)$ is related to the positional information of nodes which can be captured by the shared choice of anchor-sets.
% Together with Propositions~\ref{prop:joint_position}
%Complimentary to the discussion in Section \ref{sc:connection_to_gnns},
Thus, we conclude that P-GNNs, which embed nodes using the joint distribution of their distances to common anchors, have more expressive power than existing GNNs. 

\subsection{Complexity Analysis}
Here we discuss the complexity of neural network computation.
In P-GNNs, every node communicates with $O(\log^2 n)$ anchor-sets in a graph with $n$ nodes and $e$ edges. Suppose on average each anchor-set contains $m$ nodes, then there are $O(mn \log^2n)$ message communications in total. If we follow the exact anchor-set selection strategy, the complexity will be $O(n^2 \log^2n)$. In contrast, the number of communications is $O(n+e)$ for existing GNNs. 
In practice, we observe that the computation can be sped up by using a simplified aggregation $\textsc{Agg}_S$, while only slightly sacrificing predictive performance. 
Here for each anchor-set, we only aggregate message from the node closest to a given node $v$. This removes the factor $m$ in the complexity of P-GNNs, making the complexity $O(n\log^2n)$. 
% The complexity of P-GNN does not depend on the average degree of nodes in $G$, and thus P-GNN will be more efficient than a GNN of the graph is dense.
We use this implementation in the experiments.






















% \cut{
% Using the definition of mutual information, we show in Proposition \ref{prop:joint_betterthan_marginal} (Proof in appendix \todo{proof}) that the joint distribution of anchor distance has higher mutual information with any objective, compared to using marginal distributions.

% \begin{proposition}
% \label{prop:joint_betterthan_marginal}
% Using joint is always better than using marginal.
% The mutual information $I(Y; X_{joint})>I(Y; X_{marginal})$, where $X_{joint} = (m(v_i, S), m(v_j, S)) \sim p(m(v_i, S), m(v_j, S))$; $X_{marginal} = (m(v_i, S), m(v_j, S))$, $m(v_i, S) \sim p(m(v_i, S), m(v_j, S) \sim p(m(v_j, S)$.

% \end{proposition}


% Propositions~\ref{prop:joint_position}  show that the joint distribution $p(d_{sp}(v_i, S), d_{sp}(v_j, S))$ provides powerful node embeddings that can better capture positional information.

% Furthurmore, no fixed node ordering is used during aggregation of messages, and therefore the embedding is naturally node permutation invariant.

% Also, the anchor distance distribution can be computed for any graphs where shortest path distance can be computed. If we assume there exists an underlying objective function $d_y$ for a multi-graph dataset, the learned embedding model $f_\theta$ is inductive.
% }







% Even being simple, we show in Corollary \ref{cor:props_hold} (Proof in appendix \todo{proof}) that the results in \ref{sc:anchor_distance} still hold.

% \begin{corollary}
% \label{cor:props_hold}
% Proposition 3, 4, 5 hold when substituting $d^k_{sp}(v_i,v_j)$ with $d_{sp}(v_i,v_j)$.
% \end{corollary}

% Given Corollary \ref{cor:props_hold}, we consider using $1$ thresholded shortest path distance $d_{sp}^1$ which is essentially directly given by the edge set $E$ of the graph.












==> Position-aware Graph Neural Networks (1)/040experiments.tex <==
\section{Experiments}



% \begin{table*}[t]
% \centering
% \begin{footnotesize}
% \caption{\name compared to GNNs in link prediction and community detection task, measured in AUC.}
% \label{tab:mmd_small}
% \begin{tabular}{@{}llllllllll@{}}
% \toprule
%               & \multicolumn{6}{c}{Link prediction} & \multicolumn{3}{c}{Community detection} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-7}\cmidrule(lr){8-10}
%               & Grid-T & Cora-T  &  Grid & Cora & Communities & PPI & Communities & Email & Protein  \\ \midrule
% GAT             &- &- & $0.588 \pm 0.049$&$0.533 \pm 0.107$ &  & - & - & - & -\\
% GraphSAGE       &- &- &$0.605 \pm 0.037$ &  $0.677\pm 0.026$ &- & - & - & - & -\\
% MPNN            &- &- &$0.617 \pm 0.045$&$0.500 \pm 0$ &- & - & - & - & -\\
% GCN             & &- &$0.633 \pm 0.054$&$0.678 \pm 0.015$ & $0.589 \pm 0.024$ & - & $0.886 \pm 0.021$& $0.674 \pm 0.061$ & -\\ \midrule
% P-GNN-Fast      & - &- & $0.690 \pm 0.038$&$0.705 \pm 0.011 $&$0.669 \pm 0.058$ & - & $0.944 \pm 0.005$ & $0.712 \pm 0.095$ & -\\
% P-GNN-Fast-2Layer & - &- & $0.676 \pm 0.068$ & $0.733 \pm 0.010$ & $0.669 \pm 0.058$ & - & $0.944 \pm 0.005$ & $0.712 \pm 0.095$ & -\\\bottomrule

% P-GNN-Exact         &- &- &$0.872 \pm 0.021$&$0.850 \pm 0.011$ & $0.904 \pm 0.011$ & - & $0.944 \pm 0.005$ & $0.693 \pm 0.087$ & -\\
% P-GNN-Exact-2Layer &- &- &$0.775 \pm 0.135$&$0.855 \pm 0.005$ & $0.904 \pm 0.011$ & - & $0.944 \pm 0.005$ & $0.693 \pm 0.087$ & -\\\bottomrule

% \end{tabular}
% \end{footnotesize}
% \end{table*}








% \begin{table*}[t]
% \centering
% \begin{footnotesize}
% \caption{P-GNNs compared to GNNs in link prediction task, measured in AUC. Grid-T and Cora-T refer to the transductive learning setting of Grid and Cora, where one-hot feature vectors are used to augment the node attributes. Standard deviation errors are given.}
% \label{tab:link_pred}
% \begin{tabular}{@{}llllllllll@{}}
% \toprule
%               & Grid-T & Cora-T  &  Grid & Cora & Communities & PPI   \\ \midrule
% GAT             &$0.529 \pm 0.117$ &$0.522 \pm 0.079$ & $0.588 \pm 0.049$&$0.533 \pm 0.107$ & $0.571 \pm 0.029$  & $0.520 \pm 0.047$ \\
% GraphSAGE       &$0.647\pm 0.024$& $0.757 \pm 0.020$ &$0.605 \pm 0.037$ &  $0.677\pm 0.026$ &$0.876 \pm 0.017$& $0.673 \pm 0.011$ \\
% MPNN            &$0.628 \pm 0.041$ &$0.618 \pm 0.083$ &$0.617 \pm 0.045$&$0.557 \pm 0.035$ &$0.711 \pm 0.044$ & $0.610 \pm 0.017$ \\
% GCN             &$0.637\pm 0.020$&$0.763 \pm 0.012$ &$0.633 \pm 0.054$&$0.678 \pm 0.015$ & $0.889 \pm 0.014$ & $0.672 \pm 0.010$ \\ \midrule
% P-GNN-Fast      & $0.644\pm 0.032$ &$0.692 \pm 0.021$ & $0.690 \pm 0.038$&$0.705 \pm 0.011 $&$0.960 \pm 0.080$ & $0.629 \pm 0.015$ \\
% P-GNN-Fast-2Layer & $0.676\pm 0.034$ & $0.673 \pm 0.053$ & $0.676 \pm 0.068$ & $0.733 \pm 0.010$ & $0.918\pm 0.062$ & $\mb{0.680} \pm 0.010$ \\\midrule
% P-GNN-Exact         &$0.792\pm 0.026$ &$\mb{0.787}\pm 0.022$ & $\mb{0.872} \pm 0.021$ & $0.850 \pm 0.011$ & $\mb{0.971} \pm 0.003$ & $0.666 \pm 0.017$ \\
% P-GNN-Exact-2Layer & $\mb{0.844}\pm 0.029$ &$0.772 \pm 0.087$ &$0.775 \pm 0.135$ & $\mb{0.855} \pm 0.005$ & $0.831\pm 0.124$ & $0.674 \pm 0.009$ \\ \bottomrule

% \end{tabular}
% \vspace{-4mm}
% \end{footnotesize}
% \end{table*}



\begin{table*}[t]
\centering
\begin{footnotesize}
\caption{P-GNNs compared to GNNs on link prediction tasks, measured in ROC AUC. Grid-T and Communities-T refer to the transductive learning setting of Grid and Communities, where one-hot feature vectors are used as node attributes. Standard deviation errors are given.}
\label{tab:link_pred}
\begin{tabular}{@{}llllllllll@{}}
\toprule
               & Grid-T & Communities-T  &  Grid  & Communities & PPI   \\ \midrule
GCN             &$0.698 \pm 0.051$ &$0.981 \pm 0.004$ & $0.456 \pm 0.037$ & $0.512 \pm 0.008$  & $0.769 \pm 0.002$ \\
GraphSAGE        &$0.682 \pm 0.050$ &$0.978 \pm 0.003$ & $0.532 \pm 0.050$& $0.516 \pm  0.010$  & $0.803 \pm 0.005$ \\
GAT             &$0.704 \pm  0.050$ &$0.980 \pm 0.005$ & $0.566 \pm 0.052$& $0.618 \pm 0.025$  & $0.783 \pm 0.004$ \\
GIN              &$0.732 \pm 0.050$ &$0.984 \pm 0.005$ & $0.499 \pm 0.054$& $0.692  \pm 0.049$  & $0.782 \pm 0.010$ \\ \midrule
P-GNN-F-1L       &$0.542 \pm 0.057$ &$0.930 \pm 0.093$ & $0.619 \pm 0.080$& $0.939 \pm 0.083$  & $0.719 \pm 0.027$ \\
P-GNN-F-2L  &$0.637 \pm 0.078$ &$\mb{0.989} \pm 0.003$ & $0.694 \pm 0.066$& $\mb{0.991} \pm 0.003$  & $0.805 \pm 0.003$  \\\midrule
P-GNN-E-1L         &$0.665 \pm 0.033$ &$0.966 \pm 0.013$ & $0.879 \pm 0.039$& $0.985 \pm 0.005$  & $0.775 \pm 0.029$ \\
P-GNN-E-2L  &$\mb{0.834} \pm 0.099$ &$0.988 \pm 0.003$ & $\mb{0.940} \pm 0.027$& $0.985 \pm 0.008$  & $\mb{0.808} \pm 0.003$ \\ \bottomrule

\end{tabular}
% \vspace{-3mm}
\end{footnotesize}
\end{table*}



\begin{table}[t]
% \vspace{-2mm}
\centering
\begin{footnotesize}
\caption{Performance on pairwise node classification tasks, measured in ROC AUC. Standard deviation errors are given.}
\label{tab:community_detect}

\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}llll@{}}
\toprule
               & Communities & Email & Protein  \\ \midrule
GAT              & $0.520 \pm 0.025$ & $0.515 \pm 0.019$ & $0.515 \pm 0.002$\\
GraphSAGE      & $0.514 \pm 0.028$ & $0.511 \pm 0.016$& $0.520 \pm 0.003$\\
GAT            & $0.620 \pm 0.022$ & $0.502 \pm 0.015$ & $0.528 \pm 0.011$\\
GIN             & $0.620 \pm 0.102$& $0.545 \pm 0.012$ & $0.523 \pm 0.002$\\ \midrule
P-GNN-F-1L      & $0.985 \pm 0.008$ & $0.630 \pm 0.019$ & $0.510 \pm 0.010$\\
P-GNN-F-2L & $0.997 \pm 0.006$ & $\mb{0.640} \pm 0.037$ & $\mb{0.729} \pm 0.176$\\\midrule
P-GNN-E-1L  & $0.991 \pm 0.013$ & $0.625 \pm 0.058$ & $0.507 \pm 0.006$\\
P-GNN-E-2L & $\mb{1.0} \pm 0.001$ & $\mb{0.640} \pm 0.029$ & $0.631 \pm 0.175$\\\bottomrule

\end{tabular}}
% \vspace{-3mm}
\end{footnotesize}
\end{table}




% \begin{table}[t]
% \centering
% \begin{footnotesize}
% \caption{P-GNNs compared to GNNs in community detection task, measured in AUC. Standard deviation errors are given.}
% \label{tab:community_detect}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}llll@{}}
% \toprule
%               & Communities & Email & Protein  \\ \midrule
% GAT              & $0.658 \pm 0.031$ & $0.764 \pm 0.020$ & $0.511 \pm 0.012$\\
% GraphSAGE      & $0.833 \pm 0.006$ & $0.772 \pm 0.033$& $0.569 \pm 0.022$\\
% MPNN            & $0.681 \pm 0.018$ & $0.712 \pm 0.022$ & $0.533 \pm 0.015$\\
% GCN             & $0.801 \pm 0.004$& $0.765 \pm 0.018$ & $0.548 \pm 0.017$\\ \midrule
% P-GNN-F-1L      & $\mb{0.989} \pm 0.002$ & $0.777 \pm 0.036$ & $0.608 \pm 0.049$\\
% P-GNN-F-2L & $0.986 \pm 0.003$ & $\mb{0.889} \pm 0.024$ & $0.728 \pm 0.052$\\\midrule
% P-GNN-E-1L  & $0.983 \pm 0.001$ & $0.780 \pm 0.026$ & $0.627 \pm 0.080$\\
% P-GNN-E-2L & $0.965 \pm 0.015$ & $0.876 \pm 0.019$ & $\mb{0.757} \pm 0.062$\\\bottomrule

% \end{tabular}}
% \vspace{-7mm}
% \end{footnotesize}
% \end{table}

%Next we describe experimental results.

\subsection{Datasets}

We perform experiments on both synthetic and real datasets. We use the following datasets for a link prediction task:
\\
% \-\hspace{5mm} $\bullet$ \xhdr{Cora}
% A citation network with $|V|=2708, |E|=5429$, each node has $1433$ dimensional features.
% \\
\-\hspace{5mm} $\bullet$ \xhdr{Grid
} 2D grid graph representing a 20$\times$ 20 grid with $|V|=$ 400 and no node features. 
% Each graph has $20\%$ of edges removed uniformly at random.
\\
\-\hspace{5mm} $\bullet$ \xhdr{Communities}
Connected caveman graph \cite{watts1999networks} with 1\% edges randomly rewired, with 20 communities where each community has 20 nodes.
\\
\-\hspace{5mm} $\bullet$ \xhdr{PPI}
24 Protein-protein interaction networks \cite{zitnik2017predicting}. Each graph has 3000 nodes with avg. degree 28.8, each node has 50 dimensional feature vector.

We use the following datasets for pairwise node classification tasks which include community detection and role equivalence prediction\footnote{Inductive position-aware node classification is not well-defined due to permutation of labels in different graphs. However pairwise node classification, which only decides if nodes are of the same class, is well defined in the inductive setting.}.
\\
\-\hspace{5mm} $\bullet$ \xhdr{Communities}
The same as above-mentioned community dataset, with each node labeled with the community it belongs to.
\\
\-\hspace{5mm} $\bullet$ \xhdr{Emails}
7 real-world email communication graphs from SNAP \cite{leskovec2007graph} with no node features. Each graph has 6 communities and each node is labeled with the community it belongs to.
\\
\-\hspace{5mm} $\bullet$ \xhdr{Protein}
1113 protein graphs from \cite{borgwardt2005protein}. Each node is labeled with a functional role of the protein. Each node has a 29 dimensional feature vector.


% \xhdr{Molecules \jiaxuan{~2 hours}}
% $xx$ molecule graphs from ZINC \CITE without node or edge attributes.
% Each node is labeled with its atom type.



% \xhdr{Ego \jiaxuan{1 hours}}
% xx 3-hop ego graphs extracted from citeseer.
% Each node is labeled with its shortest path distance to the ego center, 4 classes in total.



\subsection{Experimental setup}

% \subsubsection{Learning settings}

%We show that P-GNNs perform well in both transductive and inductive learning settings.

Next we evaluate P-GNN model on both transductive and inductive learning settings.

\xhdr{Transductive learning}
In the transductive learning setting, the model is trained and tested on a given graph with a fixed node ordering and has to be re-trained whenever the node ordering is changed or a new graph is given.
As a result, the model is allowed to augment node attributes with unique one-hot identifiers to differentiate different nodes.
Specifically, we follow the experimental setting from \cite{zhang2018link}, and use two sets of 10\% existing links and an equal number of nonexistent links as test and validation sets, with the remaining 80\% existing links and equal number of nonexistent links used as the training set.
We report the test set performance when the best performance on the validation set is achieved, and we report results over 10 runs with different random seeds and train/validation splits.

\xhdr{Inductive learning}
We demonstrate the inductive learning performance of P-GNNs on pairwise node classification tasks for which it is possible to transfer the positional information to a new unseen graph.
% \footnote{For non-pairwise node classification tasks, although structure information can be transfered to unseen graphs, positional information cannot, due to permutation of position-based information.}. 
% \cut{remove:
% In the inductive learning setting, we consider two possible cases: (1) when the dataset only consists of one graph, we expect the learned model to not rely on a fixed node ordering so that it can be transfered to future test graphs; (2) when the dataset consists of multiple graphs, the model is trained on some training graphs and tested on other unseen graphs.}
In particular, for inductive tasks, augmenting node attributes with one-hot identifiers restricts a model's generalization ability, because the model needs to generalize across scenarios where node identifiers can be arbitrarily permuted.
Therefore, when the dataset does not come with node attributes, we only consider using constant order-invariant node attributes, such as a constant scalar, in our experiments. Original node attributes are used if they are available.

We follow the transductive learning setting to sample links, but only use order-invariant attributes. When multiple graphs are available, we use 80\% of the graphs for training and the remaining graphs for testing. Note that we do not allow the model to observe ground-truth graphs at the training time. 
% for realistic link prediction scenarios \cite{liben2007link}.
For the pairwise node classification task, 
% \rex{remove: node labels are transformed into pairwise labels. Instead of assigning each community an ID, which can be permuted in exponentially many ways and hard to optimize, }
we predict whether a pair of nodes belongs to the same community/class. In this case, a pair of nodes that do not belong to the same community are a negative example.
% \rex{remove: Specifically, we split $20\%$ of the graphs as the testing graphs and the remaining graphs as the training graphs. We then use all the positive pairs and sample the same number of negative pairs from the training graphs to train a model, and test over test graphs with the same sample strategy.}

\subsection{Baseline models}
So far we have shown that P-GNNs are a family of models that differ from the existing GNN models.
Therefore, we compare variants of P-GNNs against most popular GNN models. To make a fair comparison, all models are set to have similar number of parameters and are trained for the same number of epochs. We fix model configurations across all the experiments. (Implementational details are provide in the Appendix.)
% and almost all existing GNNs can be adapted to the P-GNN framework.
% Therefore, we select some typical GNN models, and adapt them \rex{remove: the common formulation Graph Convolutional Networks (GCN)} to the P-GNN framework. We show even the simplest P-GNN model can significantly outperform many GNN models\rex{remove:, and designing more expressive P-GNN models are left for the future work}. 
% For GNNs, we use the architectures that has(detailed in appendix).
We show that even the simplest P-GNN models can significantly outperform GNN models in many tasks, and designing more expressive P-GNN models is an interesting venue for future work.

\xhdr{GNN variants}
We consider 4 variants of GNNs, each with three layers, including GCN \cite{kipf2016semi}, GraphSAGE \cite{hamilton2017inductive}, Graph Attention Networks (GAT) \cite{velickovic2017graph} and Graph Isomorphism Network (GIN) \cite{xu2018powerful}. Note that in the context of link prediction task, our implementation of GCN is equivalent to GAE \cite{kipf2016variational}.
% and SEAL \cite{zhang2018link}. 
% All the models can be trained for both transductive and inductive settings except 

% Deep Graph Infomax. \jiaxuan{Code on github, if 2 hours it still doesn't work, try MPNN/GAT} 
% that paper is unsupervise learning only

\xhdr{P-GNN variants}
We consider 2 variants of P-GNNs, either with one layer or two layers (labeled 1L, 2L): (1) P-GNNs using truncated 2-hop shortest path distance (P-GNN-F); (2) P-GNNs using exact shortest path distance (P-GNN-E).


% \xhdr{Random walk models ?? \jiaxuan{not priority}}
% We use DeepWalk \jiaxuan{2 hours}, and DeepWalk + features. Note that they cannot be generalized to different graphs.

% (2) P-GNN with independent neighbourhood sampling which is equivalent to an ensemble of GraphSage models \cite{hamilton2017inductive};


\subsection{Results}

\xhdr{Link prediction}
In link prediction tasks two nodes are generally more likely to form a link, if they are close together in the graph. Therefore, the task can largely benefit from position-aware embeddings.
%In comparison, structurally similar nodes such as corners in a grid are not indicative of links, making the task challenging for GNN models that are not position-aware.
Table \ref{tab:link_pred} summarizes the performance of P-GNNs and GNNs on a link prediction task.
% \rex{The results are obtained by averaging 10 runs with different random seeds and train/validation splits.}
We observe that P-GNNs significantly outperform GNNs across all datasets and variants of the link prediction taks (inductive vs. transductive). P-GNNs perform well in all inductive link prediction settings, for example improve AUC score by up to 66\% over the best GNN model in the grid dataset.
In the transductive setting, P-GNNs and GNNs achieve comparable performance.
The explanation is that one-hot encodings of nodes help GNNs to memorize node IDs and differentiate symmetric nodes, but at the cost of expensive computation over $O(n)$ dimensional input features and the failure of generalization to unobserved graphs. On the other hand, P-GNNs can discriminate symmetric nodes by their different distances to anchor-sets, and thus adding one-hot features does not help their performance.
% GNN models can perform well in transductive settings where good performance can be achieved via memorizing nodes' unique identifiers, but they fail to perform well in inductive settings where generalizable positional information is needed.
In addition, we observe that when graphs come with rich features (e.g., PPI dataset), the performance gain of P-GNNs is smaller, because node features may already capture positional information. Quantifying how much of the positional information is already captured by the input node features is an interesting direction left for future work.
% While using the exact shortest path distance is more powerful and achieves better performances, it is computationally expensive. 
Finally, we show that the ``fast'' variant of the P-GNN model (P-GNN-F) that truncates expensive shotest distance computation at 2 still achieves comparable results in many datasets.

\xhdr{Pairwise node classification}
In pairwise node classification tasks, two nodes may belong to different communities but have similar neighbourhood structures, thus GNNs which focus on learning structure-aware embeddings will not perform well in this tasks.
Table \ref{tab:community_detect} summarizes the performance of P-GNNs and GNNs on pairwise node classification tasks. The capability of learning position-aware embeddings is crucial in the Communities dataset, where all P-GNN variants nearly perfectly detect memberships of nodes to communities, while the best GNN can only achieve 0.620 ROC AUC, which means that P-GNNs give 56\% relative improvement in ROC AUC over GNNs on this task. Similar significant performance gains are also observed in Email and Protein datasets: 18\% improvement in ROC AUC on Email and 39\% improvement of P-GNN over GNN on Protein dataset.





==> Position-aware Graph Neural Networks (1)/050conclusion.tex <==
\section{Conclusion}

We propose Position-aware Graph Neural Networks, a new class of Graph Neural Networks for computing node embeddings that incorporate node positional information, while retaining inductive capability and utilizing node features. We show that P-GNNs consistently outperform existing GNNs in a variety of tasks and datasets.

\section*{Acknowledgements}
\label{sec:ack}
This research has been supported in part by Stanford Data Science Initiative, NSF, DARPA, Boeing, Huawei, JD.com, and Chan Zuckerberg Biohub.

==> Position-aware Graph Neural Networks (1)/archive_proposed.tex <==
\section{Proposed Approach}

\jiaxuan{A figure for the model}

\subsection{Notation and Problem definition}

% notation
A graph can be represented as $G = (V,E)$, where $V = \{v_1, ..., v_n\}$ is the node set, $E=\{(v_i,v_j)|v_i,v_j\in V\}$ is the edge set. When a node has internal attributes, there may exist the node feature set $F = \{f_1, ..., f_n\}$ where $f_i$ is the feature associated with node $v_i$. For notation simplicity, we use $V$ to refer to both $V$ and $F$ if $F$ exists.



% We propose to view node- or edge-level prediction tasks within graphs as the transformation of metric spaces.
% Given a graph $G$, we can define an arbitrary metric space $S = (V, d)$, where $d(v_i, v_j)$ is a valid distance function.
% We are assumed to have observable distance function $d_x(\cdot, \cdot)$ for all pairs of the nodes, while having labeling function $d_y(\cdot, \cdot)$ whose values are only observed in training node pairs.
% A learning task can therefore be written as learning a transformation that maps $S_x = (V, d_x)$ to $S_y = (V, d_y)$.
% Note that this formulation naturally represents edge-level prediction tasks, while node classification task can be transformed to pairwise labeling function up to node class permutations. Further details are discussed in Section \ref{}.

Usually, predictions on graphs are made via learning a node embedding model. Specifically, a node embedding model can be written as a function $f: V \rightarrow Z$ that maps nodes $V$ to low-dimensional vectors $Z = \{z_1, ..., z_n\}, z_i \in \mathbb{R}^k$.
% , which implies a new metric space $S_z = (Z, d_z)$.
Node-level prediction tasks correspond to a unary objective function $d_y(v_i)$, while edge-level prediction tasks imply a pairwise objective function $d_y(v_i, v_j)$.
Learning node embedding can then be written as an optimization problem, $\min \mathbb{E}_{(v_i,v_j)\sim E_{train}}[L(d_z(z_i,z_j)-d_y(v_i,v_j))]$ for edge-level tasks, and $\min \mathbb{E}_{v_i\sim V_{train}}[L(d_z(z_i)-d_y(v_i))]$ for node-level tasks, where $L(\cdot, \cdot)$ is a loss function.
A common additional requirement is that $d_z(\cdot,\cdot)$ should be $l_2$ metric, so that the computed embeddings are interpretable and can be easily used for downstream tasks.

In this paper, we call the node embeddings to be position-aware, if the node embeddings can be used to recover the shortest path distance. This property is crucial for many prediction tasks, such as link prediction and community detection.
Specifically, let $d_{sp}(v_i,v_j)$ be the shortest path, then $d_{sp}(v_i, v_j) = g(d_z(f(v_i), f(v_j)))$ holds for position-aware node embeddings.
We will show in Section \ref{} that GNN-based embeddings cannot recover the shortest path distance between two nodes in practical settings; therefore, GNN models cannot achieve satisfactory performance in the above-mentioned prediction tasks.


The above formulation is for transductive learning settings, where models are trained and tested on the same graph. The formulation can be generalized to inductive settings that is much more practical in real-world problems.
In the inductive setting, $G$ is viewed as a sample from a class of graph $G \in \mathbb{G}$. The goal is to learn an underlying objective function $d_y$ that is share among any $G \in \mathbb{G}$, via a shared embedding model $f$ that can take any $G \in \mathbb{G}$ as input.


% Jiaxuan: we give up using the unsupervised settings, but describe in more general terms.

% The ability to preserve the distance metric can be formalized via the notion of distortion. Specifically, $f$ is defined to have distortion $\alpha$ if for all $v_i, v_j \in V$, $d(v_i, v_j) \leq d'(f(v_i), f(f_j)) \leq \alpha d(v_i, v_j)$ holds.


% problem definition




% Jiaxuan: use different way to describe the problem
% In this paper, we aim to learn inductive position-aware node embeddings. We call an embedding method to be position-aware, if the computed node embeddings $X$ can be used to precisely reconstruct the graph \jiaxuan{could say in other ways}. 
% This property implies two requirements: (1) the original distance metric $d(\cdot)$ should reflect global graph connectivity; (2) the embedding method should be able to (approximately) preserve the distance.
% As we will later show, although existing GNN-based models are trained with objectives following the first requirement, they can only preserve distance metrics that reflect structural equivalence \jiaxuan{check expression}, thus fails to generate valid position-aware node embeddings.
% In addition, we expect the embedding method to be inductive, i.e., the method does not require gaining new labels and retraining in unseen graphs.


% \subsection{GNNs fail to learn position-aware embeddings}

\subsection{Limitations of structure-aware embeddings}

We identify two types of node embeddings that are of special interests, which we name as structure-aware embeddings and position-aware embeddings.
Structure-aware embeddings detect the structural role for a given node, usually involve some approximate graph isomorphism test. 
Position-aware embeddings reflect homophily properties in the graph \cite{grover2016node2vec}, which is highly related to the shortest path distance metrics.
Usually, tasks such as community detection and link prediction require more of position-aware embeddings, while common node classification tasks reflect more of position-aware distances.
Although both types of embeddings have been used to qualitatively discuss the nature of various network prediction tasks, their relationships are not clearly understood. 
To take deeper analysis, we first define the two types of node embeddings that will be discussed throughout this paper.

\begin{definition}
A node embedding $z_i = f_p(v_i)$ is position-aware if there exists function $g(\cdot, \cdot)$ such that $d_{sp}(v_i, v_j) = g(z_i, z_j)$, where $d_{sp}(\cdot, \cdot)$ is the shortest path distance.
\end{definition}

\begin{definition}
A node embedding $z_i = f_s(v_i)$ is structure-aware if it is a function of each hop neighbourhood of node $v_i$. Specifically, $z_i = g(g_1(N_1(v_i)),...,g_q(N_q(v_i)))$, where $N_k(v_i)$ is the set of the $k$-hop neighbourhood of $v_i$, and $g, g_k, k=1,...,q$ can be any functions.

% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h_k(\cdot)(N_k(v_i))$ over the $k$-hop neighbourhoods of a node. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
\end{definition}

% \begin{definition}
% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h_k(\cdot)(N_k(v_i))$ over the $k$-hop neighbourhoods of a node. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
% \end{definition}



% \subsubsection{A spectrum of distance metrics}

% We identify two types of distance metrics $d(\cdot, \cdot)$ that are of special interests, which we name as structure-aware distances and position-aware distances.
% Structure-aware distances detect the similarity of the structural role for a given node, usually involve some approximate graph isomorphism test. 
% Position-aware distances are called as homophily similarity in the literature as well \cite{grover2016node2vec}, which is highly related to the shortest path distance.
% Usually, tasks such as community detection reflects more of position-aware distances, while general node classification tasks reflects more of structure-aware distances.
% Although both types of distances have been used to qualitatively discuss the nature of various network prediction tasks, their relationships are not clearly understood. 
% To take deeper analysis, we first define the two types of distance metrics that will be discussed throughout this paper.


% \begin{definition}
% A position-aware distance $d_p(\cdot, \cdot)$ is determined by the shortest path distance $d_{sp}(\cdot, \cdot)$, i.e., $d_p(v_i, v_j) = g(d_{sp}(v_i, v_j))$.
% \end{definition}

% \begin{definition}
% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h_k(\cdot)(N_k(v_i))$ over the $k$-hop neighbourhoods of a node. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
% \end{definition}

% \begin{definition}
% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h(\cdot)$ of a node's $k$-hop neighbourhood. $d_{iso}(N_k(v_i), N_k(v_j)) \in \{0, 1\}$, where $N_k(v_i)$ is the graph over $k$-hop neighbours of node $v_i$ \jiaxuan{should be GCN style computational graph, not sure}. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
% \end{definition}

% The dichotomy between structure-aware and position-aware distances

Based on the definitions, we point out that there is a dichotomy between structure-aware and position-aware embeddings. Specifically, structure-aware embeddings cannot reproduce position-aware embeddings in most cases.
Therefore, when the learning task requires node position information, only using structure-aware embeddings as input features is not sufficient.


% \jiaxuan{Not sure if it's good}
% \begin{proposition}
% \label{prop:dist_ortho}
% The shortest path distance $d_{sp}$ is a function of structure-aware embeddings $f_s(v_i)$, if and only $f_s(v_i)\neq f_s(v_j)$ holds for any pair of nodes.
% \end{proposition}

% \begin{proof}
% If no pairs of nodes have $d_{s_k}(v_i, v_j) = 0$, then each node can be assigned a unique identifier, then by count the $\argmin$ of the hop that $v_j$ appears in $v_i$'s neighbourhood one can get the $d_{sp}(v_i, v_j)$ which can then be used to compute $d_p(v_i, v_j)$ by definition.

% When $d_{sp}$ is a function of $d_{s_k}$, if there exists $d_{s_k}(v_i, v_j) = 0$, then for any node $v_k$ $d_{s_k}(v_i, v_k) = d_{s_k}(v_j, v_k)$, which means $d_{sp}(v_i, v_k) = d_{sp}(v_j, v_k)$ for any node $v_k$, thus $d_{sp}(v_i, v_i) = d_{sp}(v_i, v_j) = 0$. This contradict with the fact that $d_{sp}(v_i, v_j) = 1$, thus there does not exist $d_{s_k}(v_i, v_j) = 0$, which finishes the proof.
% \end{proof}


% jiaxuan: this version seems better
\begin{proposition}
\label{prop:dist_ortho}
The shortest path distance $d_{sp}$ is a function of structure-aware embeddings $f_s(v_i)$, if and only $f_s(v_i)\neq f_s(v_j)$ holds for any pair of nodes.
\end{proposition}


In real world datasets, $d_{s_k}(v_i, v_j) = 0$ rarely holds, especially when $k$ is small.
Therefore, Proposition 1 shows that position-aware metrics is usually not explainable by using structural-aware metrics.

\jiaxuan{maybe need another proposition}
As is shown in \CITE, Graph Convolutional Networks (GCNs) are equivalent of doing approximate graph isomorphism test, where $k$-layer GCNs corresponding to computing $d_{s_k}$ at best. Thus, GNN models fail to capture the position-aware component in the objective metric function $d_y(\cdot, \cdot)$. More expressive model is needed to learn the position-aware component in the object.





% In this section, we show that different prediction task implies different distance metrics over the metric space $S = (V, d)$ in the original graph. Note that only some class of distance metrics can lead to position-aware embeddings.



% \subsubsection{Examples of distance metrics}

% \xhdr{Node classification distance} Node classification task refers to classifying unseen nodes.
% $Y = \{y_1, ..., y_n\}$ is the node label set where $y_i$ is the feature associated with node $v_i$.
% The task is often trained with supervised training objective
% \begin{equation}
%     CrossEntropy(p_i, y_i)
% \end{equation}
% In some inductive learning settings, for example community detection task, the node label can be arbitrarily permuted, making the about objective problematic.
% One possible distance metric that implies the above objective while being permutation invariant is
% \begin{align}
%     & d(v_i, v_j) = 0, \text{if } y_i = y_j \\
%     & d(v_i, v_j) = 1, \text{otherwise}
% \end{align}

% \xhdr{binary shortest path distance}
% One possible distance metric that implies the above objective is 
% \begin{align}
%     & d(v_i, v_j) = 1, \text{if } (v_i, v_j) \in E_{train} \\
%     & d(v_i, v_j) = 2, \text{otherwise}
% \end{align}
% Lemma: this distance metric is valid.


% \xhdr{Link prediction based distance}
% Link prediction task often refers to predicting missing edges within a graph.
% A common objective is to force connected nodes to have similar embeddings while disconnected nodes should have distant embeddings. Specifically, a widely adopted objective \cite{hamilton2017inductive} is
% \begin{equation}
%     J(\mathbf{z}_u) = -\log(\sigma(\mathbf{z}_u^T\mathbf{z}_v)) - Q \mathbb{E}_{v_n\sim P_n(v)}\log(-\sigma(\mathbf{z}_u^T\mathbf{z}_v))
% \end{equation}
% One possible distance metric that implies the above objective is 
% \begin{align}
%     & d(v_i, v_j) = 1, \text{if } (v_i, v_j) \in E_{all} \\
%     & d(v_i, v_j) = 2, \text{otherwise}
% \end{align}
% Lemma: this distance metric is valid.



\subsection{Structure-award embeddings via random anchors}


\subsubsection{Low-distortion metric embedding method}
Discuss Bourgain theorem

\begin{theorem}
Bourgain theorem
\end{theorem}
Points out GNN only compute feature based distance.

\subsection{Embedding nodes via anchors}

Inspiration from the Bourgain Theorem, we further claim that a node can be uniquely identified using position-aware distances to randomly chosen anchors.
Specifically, a node $v_i$ can be represented by the distribution $p_{v_i} = d_p(v_i, S^Q)$, where $S^q$ is a randomly chosen anchor with probability $q$.



\subsection{DeepBourgain}
Inspired by the low-distortion metric embedding, we propose DeepBourgain that is able to generate position-aware node embeddings.


Computing DeepBourgain embedding involves three stages

\subsubsection{Anchor selection}

\subsubsection{Compute Distances}

\subsubsection{Anchor aggregation}




\subsection{Connection to GNN}
GNN are special cases of DeepBourgain.
It can be view as DeepBourgain that selects all nodes as anchors, and adopt link prediction distance.















% Another view is that we alter the neighbourhood definition in GNNs as randomly chosen anchors that are shared across all the nodes.\rex{to move later}

% \begin{algorithm}[h!]
% \caption{\textsc{P-GNN}}
% \label{alg:pgnn}
% \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \Input{ Current node $u$; set of anchor-sets $\{S_i | i \in [1, k]\}$, set of node features $\{f_i | i \in [1, n]\}$;
% distance function $d(\cdot, \cdot)$, anchor-set aggregation function $\textsc{Agg}_S(S_i)$, neighborhood aggregation function $\textsc{Agg}_N$}
% \Output{ Embedding $\mb{z}_u$ for node $u$}
%  \BlankLine
%  \For {$l=1,...,L$} {
%   \For {$S = S_1, S_2, ..., S_k$} {
%       $m_S \leftarrow d(S, u) \cdot \textsc{Agg}_S(S,v) $
%   }
%   $\mathbf{h}_{\mathcal{N}(u)}^l \rightarrow \textsc{Agg}_N(\{m_{S_i} | i \in [1, k]\})$\;\\
%   $\mb{h}_u^l \rightarrow \textrm{ReLU}\left(  W \cdot \textsc{Concat}(\mb{h}^{l-1}, \mb{h}_{\mathcal{N}(u)}^l) + \mathbf{b} \right)$\;
%  }
%  $\mb{z}_u \rightarrow \mb{h}_u^L$
% \end{algorithm}


% \begin{algorithm}[h!]
% \caption{\textsc{P-GNN}}
% \label{alg:pgnn}
% \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \Input{Graph $G=(V,E)$; set of anchor-sets $\{S_1,...,S_k\}$; input features $\{\mathbf{x}_v, \forall v \in \mathcal{V}\}$;
% distance function $d(\cdot, \cdot)$; set aggregation function $\textsc{Agg}_S(\cdot)$, $\textsc{Agg}_N(\cdot)$; non-linearity $\sigma(\cdot)$}
% \Output{Position-aware embeddings $\mb{m}_v$, structure-aware embeddings $\mb{h}_v, \forall v \in V$}
% \BlankLine
% $\mathbf{h}_v^{0} \leftarrow \mathbf{x}_v, \forall v \in V$ \\
% \For {$l=1,...,L$} {
%     \For {$v \in V$} { 
%         $\mb{m}_v^l = \mb{0} \in \mb{R}^k$ \\
%         \For {$i = 1,...,k$} {
%             $\mb{m}_v^l[i] \leftarrow \textsc{Agg}_S(\{d(v,u) \cdot \mathbf{h}_u^{l-1}, \forall u \in S_i\})$\\
%         }
%         $\mb{h}_{\mathcal{N}(v)}^l \leftarrow \textsc{Agg}_N(\{\mb{m}_v^l[i], i=1,...,k\})$\\
%         $\mb{h}_v^l \leftarrow \sigma\left(\mb{W}^l \cdot \textsc{Concat}(\mb{h}_v^{l-1}, \mb{h}_{\mathcal{N}(v)}^l)\right)$\\
%  }
%  }
%  $\mb{m}_v \leftarrow \mb{m}_v^L$ \\
%  $\mb{h}_v \leftarrow \mb{h}_v^L$ \\
% \end{algorithm}

==> Position-aware Graph Neural Networks (1)/micro.tex <==
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}
\usepackage{url}
\usepackage{verbatim} % allows multiline comments
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{caption} 
\usepackage{multirow}
%\usepackage{algorithm}
%\usepackage[noend]{algorithmic}
% \usepackage[linesnumbered,ruled]{algorithm2e}
\usepackage{xspace}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{times}
\usepackage{xr}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{hyperref}       % hyperlinks

\newcommand{\note}[1]{{{\textcolor{blue}{[note: #1]}}}}
\newcommand{\jure}[1]{{{\textcolor{red}{[Jure: #1]}}}}
\newcommand{\rex}[1]{{{\textcolor{magenta}{[Rex: #1]}}}}
\newcommand{\will}[1]{{{\textcolor{orange}{[Will: #1]}}}}
\newcommand{\xiang}[1]{{{\textcolor{cyan}{[Xiang: #1]}}}}
\newcommand{\jiaxuan}[1]{{{\textcolor{green}{[Jiaxuan: #1]}}}}

\newcommand{\xhdr}[1]{{\noindent\bfseries #1}.}
\newcommand{\todo}[1]{{\textcolor{red}{TODO: #1}}}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\CITE}{{\textcolor{red}{[CITE]}}}
\newcommand{\name}{P-GNN\xspace}

\newcommand{\V}{\mathcal{V}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\G}{\mathcal{G}}


\newcommand{\nedge}{k}
\newcommand{\mb}{\mathbf}
\newcommand{\cut}[1]{}
%\newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1}}}
\newcommand{\casc}{{\mathbf{t}}}
\newcommand{\alphs}{{\mathbf{A}}}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{observation}{\textbf{Observation}}
\newcommand{\xsketch}{\noindent {\it Proof Sketch.}}
\newcommand{\netinf}{{\textsc{Net\-Inf}}\xspace}
\newcommand{\multitree}{{\textsc{Multi\-Tree}}\xspace}
\newcommand{\netrate}{{\textsc{Net\-Rate}}\xspace}
\newcommand{\connie}{{\textsc{Co\-nNIe}}\xspace}
\newcommand{\maxinf}{{\textsc{Max\-Inf}}\xspace}
\newcommand{\expo}{{\textsc{Exp}}\xspace}
\newcommand{\pow}{{\textsc{Pow}}\xspace}
\newcommand{\ray}{{\textsc{Ray}}\xspace}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\unobs}{{\infty}}
\newcommand\T{\rule{0pt}{2.6ex}}
\newcommand\B{\rule[-1.2ex]{0pt}{0pt}}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\ba}{Barab\'asi-Albert }
\newcommand{\er}{Erd\H{o}s-R\'enyi}
\newcommand{\angstrom}{\textup{\AA}}
\newcommand{\mmd}{\mathrm{MMD}}
\newcommand{\graphrnnmlp}{GraphRNN-S}
\newcommand{\graphrnnrnn}{GraphRNN}


==> archive_proposed.tex <==
\section{Proposed Approach}

\jiaxuan{A figure for the model}

\subsection{Notation and Problem definition}

% notation
A graph can be represented as $G = (V,E)$, where $V = \{v_1, ..., v_n\}$ is the node set, $E=\{(v_i,v_j)|v_i,v_j\in V\}$ is the edge set. When a node has internal attributes, there may exist the node feature set $F = \{f_1, ..., f_n\}$ where $f_i$ is the feature associated with node $v_i$. For notation simplicity, we use $V$ to refer to both $V$ and $F$ if $F$ exists.



% We propose to view node- or edge-level prediction tasks within graphs as the transformation of metric spaces.
% Given a graph $G$, we can define an arbitrary metric space $S = (V, d)$, where $d(v_i, v_j)$ is a valid distance function.
% We are assumed to have observable distance function $d_x(\cdot, \cdot)$ for all pairs of the nodes, while having labeling function $d_y(\cdot, \cdot)$ whose values are only observed in training node pairs.
% A learning task can therefore be written as learning a transformation that maps $S_x = (V, d_x)$ to $S_y = (V, d_y)$.
% Note that this formulation naturally represents edge-level prediction tasks, while node classification task can be transformed to pairwise labeling function up to node class permutations. Further details are discussed in Section \ref{}.

Usually, predictions on graphs are made via learning a node embedding model. Specifically, a node embedding model can be written as a function $f: V \rightarrow Z$ that maps nodes $V$ to low-dimensional vectors $Z = \{z_1, ..., z_n\}, z_i \in \mathbb{R}^k$.
% , which implies a new metric space $S_z = (Z, d_z)$.
Node-level prediction tasks correspond to a unary objective function $d_y(v_i)$, while edge-level prediction tasks imply a pairwise objective function $d_y(v_i, v_j)$.
Learning node embedding can then be written as an optimization problem, $\min \mathbb{E}_{(v_i,v_j)\sim E_{train}}[L(d_z(z_i,z_j)-d_y(v_i,v_j))]$ for edge-level tasks, and $\min \mathbb{E}_{v_i\sim V_{train}}[L(d_z(z_i)-d_y(v_i))]$ for node-level tasks, where $L(\cdot, \cdot)$ is a loss function.
A common additional requirement is that $d_z(\cdot,\cdot)$ should be $l_2$ metric, so that the computed embeddings are interpretable and can be easily used for downstream tasks.

In this paper, we call the node embeddings to be position-aware, if the node embeddings can be used to recover the shortest path distance. This property is crucial for many prediction tasks, such as link prediction and community detection.
Specifically, let $d_{sp}(v_i,v_j)$ be the shortest path, then $d_{sp}(v_i, v_j) = g(d_z(f(v_i), f(v_j)))$ holds for position-aware node embeddings.
We will show in Section \ref{} that GNN-based embeddings cannot recover the shortest path distance between two nodes in practical settings; therefore, GNN models cannot achieve satisfactory performance in the above-mentioned prediction tasks.


The above formulation is for transductive learning settings, where models are trained and tested on the same graph. The formulation can be generalized to inductive settings that is much more practical in real-world problems.
In the inductive setting, $G$ is viewed as a sample from a class of graph $G \in \mathbb{G}$. The goal is to learn an underlying objective function $d_y$ that is share among any $G \in \mathbb{G}$, via a shared embedding model $f$ that can take any $G \in \mathbb{G}$ as input.


% Jiaxuan: we give up using the unsupervised settings, but describe in more general terms.

% The ability to preserve the distance metric can be formalized via the notion of distortion. Specifically, $f$ is defined to have distortion $\alpha$ if for all $v_i, v_j \in V$, $d(v_i, v_j) \leq d'(f(v_i), f(f_j)) \leq \alpha d(v_i, v_j)$ holds.


% problem definition




% Jiaxuan: use different way to describe the problem
% In this paper, we aim to learn inductive position-aware node embeddings. We call an embedding method to be position-aware, if the computed node embeddings $X$ can be used to precisely reconstruct the graph \jiaxuan{could say in other ways}. 
% This property implies two requirements: (1) the original distance metric $d(\cdot)$ should reflect global graph connectivity; (2) the embedding method should be able to (approximately) preserve the distance.
% As we will later show, although existing GNN-based models are trained with objectives following the first requirement, they can only preserve distance metrics that reflect structural equivalence \jiaxuan{check expression}, thus fails to generate valid position-aware node embeddings.
% In addition, we expect the embedding method to be inductive, i.e., the method does not require gaining new labels and retraining in unseen graphs.


% \subsection{GNNs fail to learn position-aware embeddings}

\subsection{Limitations of structure-aware embeddings}

We identify two types of node embeddings that are of special interests, which we name as structure-aware embeddings and position-aware embeddings.
Structure-aware embeddings detect the structural role for a given node, usually involve some approximate graph isomorphism test. 
Position-aware embeddings reflect homophily properties in the graph \cite{grover2016node2vec}, which is highly related to the shortest path distance metrics.
Usually, tasks such as community detection and link prediction require more of position-aware embeddings, while common node classification tasks reflect more of position-aware distances.
Although both types of embeddings have been used to qualitatively discuss the nature of various network prediction tasks, their relationships are not clearly understood. 
To take deeper analysis, we first define the two types of node embeddings that will be discussed throughout this paper.

\begin{definition}
A node embedding $z_i = f_p(v_i)$ is position-aware if there exists function $g(\cdot, \cdot)$ such that $d_{sp}(v_i, v_j) = g(z_i, z_j)$, where $d_{sp}(\cdot, \cdot)$ is the shortest path distance.
\end{definition}

\begin{definition}
A node embedding $z_i = f_s(v_i)$ is structure-aware if it is a function of each hop neighbourhood of node $v_i$. Specifically, $z_i = g(g_1(N_1(v_i)),...,g_q(N_q(v_i)))$, where $N_k(v_i)$ is the set of the $k$-hop neighbourhood of $v_i$, and $g, g_k, k=1,...,q$ can be any functions.

% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h_k(\cdot)(N_k(v_i))$ over the $k$-hop neighbourhoods of a node. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
\end{definition}

% \begin{definition}
% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h_k(\cdot)(N_k(v_i))$ over the $k$-hop neighbourhoods of a node. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
% \end{definition}



% \subsubsection{A spectrum of distance metrics}

% We identify two types of distance metrics $d(\cdot, \cdot)$ that are of special interests, which we name as structure-aware distances and position-aware distances.
% Structure-aware distances detect the similarity of the structural role for a given node, usually involve some approximate graph isomorphism test. 
% Position-aware distances are called as homophily similarity in the literature as well \cite{grover2016node2vec}, which is highly related to the shortest path distance.
% Usually, tasks such as community detection reflects more of position-aware distances, while general node classification tasks reflects more of structure-aware distances.
% Although both types of distances have been used to qualitatively discuss the nature of various network prediction tasks, their relationships are not clearly understood. 
% To take deeper analysis, we first define the two types of distance metrics that will be discussed throughout this paper.


% \begin{definition}
% A position-aware distance $d_p(\cdot, \cdot)$ is determined by the shortest path distance $d_{sp}(\cdot, \cdot)$, i.e., $d_p(v_i, v_j) = g(d_{sp}(v_i, v_j))$.
% \end{definition}

% \begin{definition}
% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h_k(\cdot)(N_k(v_i))$ over the $k$-hop neighbourhoods of a node. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
% \end{definition}

% \begin{definition}
% A $k$-hop structure-aware distance $d_{s_k}(v_i, v_j)$ is determined by the the function $h(\cdot)$ of a node's $k$-hop neighbourhood. $d_{iso}(N_k(v_i), N_k(v_j)) \in \{0, 1\}$, where $N_k(v_i)$ is the graph over $k$-hop neighbours of node $v_i$ \jiaxuan{should be GCN style computational graph, not sure}. Specifically, $d_{s_k}(v_i, v_j) = g(d_{iso}(N_k(v_i), N_k(v_j)))$.
% \end{definition}

% The dichotomy between structure-aware and position-aware distances

Based on the definitions, we point out that there is a dichotomy between structure-aware and position-aware embeddings. Specifically, structure-aware embeddings cannot reproduce position-aware embeddings in most cases.
Therefore, when the learning task requires node position information, only using structure-aware embeddings as input features is not sufficient.


% \jiaxuan{Not sure if it's good}
% \begin{proposition}
% \label{prop:dist_ortho}
% The shortest path distance $d_{sp}$ is a function of structure-aware embeddings $f_s(v_i)$, if and only $f_s(v_i)\neq f_s(v_j)$ holds for any pair of nodes.
% \end{proposition}

% \begin{proof}
% If no pairs of nodes have $d_{s_k}(v_i, v_j) = 0$, then each node can be assigned a unique identifier, then by count the $\argmin$ of the hop that $v_j$ appears in $v_i$'s neighbourhood one can get the $d_{sp}(v_i, v_j)$ which can then be used to compute $d_p(v_i, v_j)$ by definition.

% When $d_{sp}$ is a function of $d_{s_k}$, if there exists $d_{s_k}(v_i, v_j) = 0$, then for any node $v_k$ $d_{s_k}(v_i, v_k) = d_{s_k}(v_j, v_k)$, which means $d_{sp}(v_i, v_k) = d_{sp}(v_j, v_k)$ for any node $v_k$, thus $d_{sp}(v_i, v_i) = d_{sp}(v_i, v_j) = 0$. This contradict with the fact that $d_{sp}(v_i, v_j) = 1$, thus there does not exist $d_{s_k}(v_i, v_j) = 0$, which finishes the proof.
% \end{proof}


% jiaxuan: this version seems better
\begin{proposition}
\label{prop:dist_ortho}
The shortest path distance $d_{sp}$ is a function of structure-aware embeddings $f_s(v_i)$, if and only $f_s(v_i)\neq f_s(v_j)$ holds for any pair of nodes.
\end{proposition}


In real world datasets, $d_{s_k}(v_i, v_j) = 0$ rarely holds, especially when $k$ is small.
Therefore, Proposition 1 shows that position-aware metrics is usually not explainable by using structural-aware metrics.

\jiaxuan{maybe need another proposition}
As is shown in \CITE, Graph Convolutional Networks (GCNs) are equivalent of doing approximate graph isomorphism test, where $k$-layer GCNs corresponding to computing $d_{s_k}$ at best. Thus, GNN models fail to capture the position-aware component in the objective metric function $d_y(\cdot, \cdot)$. More expressive model is needed to learn the position-aware component in the object.





% In this section, we show that different prediction task implies different distance metrics over the metric space $S = (V, d)$ in the original graph. Note that only some class of distance metrics can lead to position-aware embeddings.



% \subsubsection{Examples of distance metrics}

% \xhdr{Node classification distance} Node classification task refers to classifying unseen nodes.
% $Y = \{y_1, ..., y_n\}$ is the node label set where $y_i$ is the feature associated with node $v_i$.
% The task is often trained with supervised training objective
% \begin{equation}
%     CrossEntropy(p_i, y_i)
% \end{equation}
% In some inductive learning settings, for example community detection task, the node label can be arbitrarily permuted, making the about objective problematic.
% One possible distance metric that implies the above objective while being permutation invariant is
% \begin{align}
%     & d(v_i, v_j) = 0, \text{if } y_i = y_j \\
%     & d(v_i, v_j) = 1, \text{otherwise}
% \end{align}

% \xhdr{binary shortest path distance}
% One possible distance metric that implies the above objective is 
% \begin{align}
%     & d(v_i, v_j) = 1, \text{if } (v_i, v_j) \in E_{train} \\
%     & d(v_i, v_j) = 2, \text{otherwise}
% \end{align}
% Lemma: this distance metric is valid.


% \xhdr{Link prediction based distance}
% Link prediction task often refers to predicting missing edges within a graph.
% A common objective is to force connected nodes to have similar embeddings while disconnected nodes should have distant embeddings. Specifically, a widely adopted objective \cite{hamilton2017inductive} is
% \begin{equation}
%     J(\mathbf{z}_u) = -\log(\sigma(\mathbf{z}_u^T\mathbf{z}_v)) - Q \mathbb{E}_{v_n\sim P_n(v)}\log(-\sigma(\mathbf{z}_u^T\mathbf{z}_v))
% \end{equation}
% One possible distance metric that implies the above objective is 
% \begin{align}
%     & d(v_i, v_j) = 1, \text{if } (v_i, v_j) \in E_{all} \\
%     & d(v_i, v_j) = 2, \text{otherwise}
% \end{align}
% Lemma: this distance metric is valid.



\subsection{Structure-award embeddings via random anchors}


\subsubsection{Low-distortion metric embedding method}
Discuss Bourgain theorem

\begin{theorem}
Bourgain theorem
\end{theorem}
Points out GNN only compute feature based distance.

\subsection{Embedding nodes via anchors}

Inspiration from the Bourgain Theorem, we further claim that a node can be uniquely identified using position-aware distances to randomly chosen anchors.
Specifically, a node $v_i$ can be represented by the distribution $p_{v_i} = d_p(v_i, S^Q)$, where $S^q$ is a randomly chosen anchor with probability $q$.



\subsection{DeepBourgain}
Inspired by the low-distortion metric embedding, we propose DeepBourgain that is able to generate position-aware node embeddings.


Computing DeepBourgain embedding involves three stages

\subsubsection{Anchor selection}

\subsubsection{Compute Distances}

\subsubsection{Anchor aggregation}




\subsection{Connection to GNN}
GNN are special cases of DeepBourgain.
It can be view as DeepBourgain that selects all nodes as anchors, and adopt link prediction distance.















% Another view is that we alter the neighbourhood definition in GNNs as randomly chosen anchors that are shared across all the nodes.\rex{to move later}

% \begin{algorithm}[h!]
% \caption{\textsc{P-GNN}}
% \label{alg:pgnn}
% \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \Input{ Current node $u$; set of anchor-sets $\{S_i | i \in [1, k]\}$, set of node features $\{f_i | i \in [1, n]\}$;
% distance function $d(\cdot, \cdot)$, anchor-set aggregation function $\textsc{Agg}_S(S_i)$, neighborhood aggregation function $\textsc{Agg}_N$}
% \Output{ Embedding $\mb{z}_u$ for node $u$}
%  \BlankLine
%  \For {$l=1,...,L$} {
%   \For {$S = S_1, S_2, ..., S_k$} {
%       $m_S \leftarrow d(S, u) \cdot \textsc{Agg}_S(S,v) $
%   }
%   $\mathbf{h}_{\mathcal{N}(u)}^l \rightarrow \textsc{Agg}_N(\{m_{S_i} | i \in [1, k]\})$\;\\
%   $\mb{h}_u^l \rightarrow \textrm{ReLU}\left(  W \cdot \textsc{Concat}(\mb{h}^{l-1}, \mb{h}_{\mathcal{N}(u)}^l) + \mathbf{b} \right)$\;
%  }
%  $\mb{z}_u \rightarrow \mb{h}_u^L$
% \end{algorithm}


% \begin{algorithm}[h!]
% \caption{\textsc{P-GNN}}
% \label{alg:pgnn}
% \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \Input{Graph $G=(V,E)$; set of anchor-sets $\{S_1,...,S_k\}$; input features $\{\mathbf{x}_v, \forall v \in \mathcal{V}\}$;
% distance function $d(\cdot, \cdot)$; set aggregation function $\textsc{Agg}_S(\cdot)$, $\textsc{Agg}_N(\cdot)$; non-linearity $\sigma(\cdot)$}
% \Output{Position-aware embeddings $\mb{m}_v$, structure-aware embeddings $\mb{h}_v, \forall v \in V$}
% \BlankLine
% $\mathbf{h}_v^{0} \leftarrow \mathbf{x}_v, \forall v \in V$ \\
% \For {$l=1,...,L$} {
%     \For {$v \in V$} { 
%         $\mb{m}_v^l = \mb{0} \in \mb{R}^k$ \\
%         \For {$i = 1,...,k$} {
%             $\mb{m}_v^l[i] \leftarrow \textsc{Agg}_S(\{d(v,u) \cdot \mathbf{h}_u^{l-1}, \forall u \in S_i\})$\\
%         }
%         $\mb{h}_{\mathcal{N}(v)}^l \leftarrow \textsc{Agg}_N(\{\mb{m}_v^l[i], i=1,...,k\})$\\
%         $\mb{h}_v^l \leftarrow \sigma\left(\mb{W}^l \cdot \textsc{Concat}(\mb{h}_v^{l-1}, \mb{h}_{\mathcal{N}(v)}^l)\right)$\\
%  }
%  }
%  $\mb{m}_v \leftarrow \mb{m}_v^L$ \\
%  $\mb{h}_v \leftarrow \mb{h}_v^L$ \\
% \end{algorithm}
